Shifting More Attention to Visual Backbone: Query-modulated Refinement Networks for End-to-End Visual Grounding

Visual grounding focuses on establishing fine-grained alignment between vision and natural language, which has essential applications in multimodal reasoning systems. Existing methods use pre-trained query-agnostic visual backbones to extract visual feature maps independently without considering the query information. We argue that the visual features extracted from the visual backbones and the features really needed for multimodal reasoning are inconsistent. One reason is that there are differences between pre-training tasks and visual grounding. Moreover, since the backbones are query-agnostic, it is difficult to completely avoid the inconsistency issue by training the visual backbone end-to-end in the visual grounding framework. In this paper, we propose a Query-modulated Refinement Network (QRNet) to address the inconsistent issue by adjusting intermediate features in the visual backbone with a novel Query-aware Dynamic Attention (QD-ATT) mechanism and query-aware multiscale fusion. The QD-ATT can dynamically compute query-dependent visual attention at the spatial and channel levels of the feature maps produced by the visual backbone. We apply the QRNet to an end-to-end visual grounding framework. Extensive experiments show that the proposed method outperforms state-of-the-art methods on five widely used datasets.

==> 1.intro._backup_20211117.tex <==
%
%In recent years, visual grounding is becoming an integral component of Vision-Language frameworks.
%
%By modeling the semantic alignments across vision and language, visual grounding framework can benefit 
%
%Given an image and a , it can .
%
Visual grounding~\cite{mao2016generation,yu2016modeling,kazemzadeh2014referitgame,plummer2015flickr30k}, i.e., localizing the referent object in an image according to the given natural language query,
is a fundamental component of multimodal reasoning system.
%
%multi-modal understanding system by returning a bounding box
%
Compared with conventional object detection methods~\cite{ren2015faster,redmon2018yolov3} which 
can only recognize the restricted categories contained in the training data,
visual grounding has the advantage of detecting novel combinations of
categories and attributes expressed in free-form text.
%
In recent years, it has attracted much attention in the field of computer vision and machine learning due to its potential applications in many 
%downstream tasks
downstream tasks, such as visual question answering~\cite{zhu2016visual7w,gan2017vqs,wang2020general}, visually-grounded language navigation~\cite{anderson2018vision,vogel2010learning} and image captioning~\cite{you2016image,anderson2018bottom,chen2020say}.
%\begin{figure}
%\centering
%\begin{subfigure}[h]{1\linewidth}
%    \includegraphics[width=1\linewidth]{title_1_cropped.pdf}
%\end{subfigure}\vspace{0.05\linewidth}
%\begin{subfigure}[h]{1\linewidth}
%    \includegraphics[width=1\linewidth]{title_2_cropped.pdf}
%\end{subfigure}
%\caption{Upper: a typical visual grounding framework that uses two individual backbones to extract visual and textual features and perform cross-modal interaction. Below: our textual information infused visual grounding framework. Before the interaction, it first extracts the textual feature as guidance and guides the visual feature extraction.}
%\end{figure}
\begin{figure}[t]
\centering
\includegraphics[width=1\linewidth]{figs/title_3_cropped.pdf}
\caption{(a) a typical end-to-end visual grounding framework that uses two individual encoders to extract visual and textual features and perform cross-modal interaction. (b) our visual grounding framewokr based on a \NetworkName.}
\label{fig:title}
\end{figure}

%Most conventional methods for visual grounding rely on a vision backbone.
%
The early methods of visual grounding focus on extending
the popularly used one-stage and two-stage object detection architectures.
%
%to achieve this goal.
%
One-stage methods~\cite{yang2020improving,ye2021one,deng2021transvg,huang2021look} use a pre-trained fully convolutional network (e.g. Darknet53~\cite{redmon2018yolov3}, ResNet~\cite{he2016deep}) to directly extract pixel-level feature maps and leverage manually-defined dense anchors to return the most likely candidate for the query text.
%
These methods are easy and efficient for learning or inference, but they cannot perform well on complex queries that have various objects and relations.
%
Two-stage methods~\cite{yang2019dynamic,yang2020graph,yu2018mattnet} use an off-the-shelf detector (e.g. Faster R-CNN~\cite{ren2015faster}) to extract the region proposals and return the one that best matches the query text using the modality-shared representations.
%
%In contrast, 
%
These methods always have better performance than the one-stage ones by introducing more complicated multimodal fusion and reasoning mechanisms~\cite{yang2019dynamic,yang2020graph,mu2021disentangled}.
%
However, the complicated fusion modules
cannot be jointly learned with the backbone of the detectors, which may
limit their ability in
multimodal
reasoning.
%
%To address this problem,
%the 
More recently,
Transformer~\cite{vaswani2017attention} has been applied in visual grounding~\cite{deng2021transvg,kamath2021mdetr} to conduct the multimodal reasoning in a more succinct manner based on pixel-level feature maps without region proposals or dense anchors.
%
%
%by comprehensively considering the visual and text features.

%However, the vision backbone is query-agnostic, which leads to many irrelevant regions or visual signals being extracted. As shown in \Cref{fig:title}(a), the extracted feature has a bias towards the detection task, which is sensitive to all salient objects, and most of them are irrelevant to the input query. Besides, the extracted feature is suitable for the pretraining classification task, which ignores the attribute and relationship, hinders the multi-modal interaction and limits localization accuracy. Moreover, the pre-trained backbone tends to extract features with different scales at specific layers, which benefits the detection task. However, in visual grounding, we only need to detect one object corresponding to the query. Existing methods use the feature map from the last layer or a query-agnostic multi-scale fusion(e.g., feature pyramid network) whose scale may be inconsistent with the referent object or be noisy. We call these two kinds of weakness semantic inconsistency and scale inconsistency. %感觉还需要进一步讨论视觉预训练会关注图像中大多数的物体，且由于用分类任务训练，对特征的抽取被局限在类比上，与开放域的任意文本对齐很困难。

%
Although existing visual grounding methods, especially the Transformer-based methods~\cite{deng2021transvg,kamath2021mdetr},
have achieved promising results,
we argue that they do not pay enough attention to the visual backbone which plays a crucial role in effective multimodal reasoning.
%
Since the visual backbone determines whether all integral visual content in the image is successfully extracted for matching the query text.
%
Currently, the most widely used backbones are the CNN model (e.g., ResNet~\cite{he2016deep}) pre-trained for image classification on ImageNet and the detector (e.g., Faster R-CNN~\cite{ren2015faster} and Mask R-CNN~\cite{he2017mask}) pre-trained for general object detection of close-set categories.
%
Therefore, the difference between the visual grounding task and the pre-training task of the backbones may lead to an {\bf inconsistency} between the visual features produced by the backbones and the ones really needed for the multimodal reasoning.
%
%with the query text.
%
As shown in \Cref{fig:title}(a), the pre-trained visual backbone is sensitive to regions that may contain the objects of pre-defined categories.
%
Whereas, the visual grounding requires the backbone to localize a different object referred to by the query.
%
A straightforward way to alleviate the inconsistency is learning the visual grounding model in an end-to-end form as in~\cite{deng2021transvg}.
%
%However, it is difficult to effectively fine-tune the query-agnostic backbone with only the supervision of the end task of object localization conditioned on the complex query text.
%{\color{red}
However, even the visual backbone can be trained end-to-end, it still cannot completely avoid the inconsistency because the backbone is query-agnostic. In other words, given the same image, the query-agnostic backbone will always output the same feature map no matter what the query sentences are during inference.
%} %我感觉之前的说法不太准确 像是说我们提出了新的supervision去训练backbone 我想把更本质的问题强调出来 然后下面
%

%
In this paper, we propose a Query-aware Dynamic Attention (\AttentionName) mechanism to address the {\bf inconsistency} issue by guiding the visual backbone.
%
%
As shown in \Cref{fig:title}(b), we guide the visual backbone with the query text by adjusting its attention distribution to %keep the visual feature space and 
extract query-consistent features,
%
%The high-quality feature map 
which benefit the cross-modal alignment between the query and the relevant region to make a correct prediction.
%
%To this end, we propose a novel asymmetric cross-modal interaction module called Query-aware Dynamic Attention to refine the visual feature map.
%
%The basic module does not simply fuse the visual and textual modality.
%
%Instead, 
%
More specifically, based on feature maps produced by the backbone, the \AttentionName\ predicts the attentions along the spatial and channel dimensions by an efficient dynamic linear layer.% where part of the parameters are generated from the query text by a trainable mapping function. % Ye 这段太长了 感觉后面这个简化一下比较好
%
Then, the spatial and channel attentions are multiplied with the original feature maps to obtain the query-consistent feature maps.
%
%
%it builds linear layers whose parameters are computed from the query's textual features.
%The text-dependent layers are applied to the visual feature to produce spatial and channel visual attention maps to reduce spatial and semantic inconsistencies, respectively.
%
%


%
We instantiate the proposed \AttentionName\ by incorporating it in the visual backbone of Swin-Transformer~\cite{liu2021Swin}, i.e., 
%to a modulated vision backbone 
stacking the \AttentionName\ module after the Transformer block at each stage of the Swin-Transformer.
%
We refer the improved visual backbone as \NetworkName\ (\ModelName).
%
To comprehensively consider the fine-grained visual features of the candidate regions at different scales,
the \ModelName\ aggregates the multiscale feature maps produced at different stages as the final output of the visual backbone.
%
%incorporating proposed Query-aware Dynamic Attention to refine its feature extraction and multiscale fusion process.
%
Finally,
we build a flexible visual grounding framework based on the recently proposed TransVG~\cite{deng2021transvg} by simply replacing the visual backbone with the proposed \ModelName.
%

The complete pipeline significantly outperforms existing methods, e.g., TransVG~\cite{deng2021transvg} (3.88\% on ReferItGame and 2.85\% on Flickr30K Entities).
%%%YXS: add examples of the specific results for the improvement.
%
Note that the proposed \AttentionName\ can be easily applied to other pre-trained visual backbones, e.g.,
%ViT\cite{dosovitskiy2020image},
ResNet~\cite{he2016deep}.

%%%YXS: this sentence needs experiment results for support.
%











%between the  that can be trained end-to-end and only requires fine-tuning with in-domain datasets like most visual grounding models.
%
%
%Experiments on various common used phrase grounding and referring expression grounding datasets demonstrate the significant performance gains of the proposed modules.
%

%

%

%

%

The main contributions of this paper are three-fold:
\begin{itemize}
%
\item 
We propose a novel query-aware dynamic attention mechanism to mitigate the inconsistency issue of the pre-trained visual backbone, which can guide the visual backbone to extract query-consistent feature maps by dynamically computing the spatial and channel attentions according to the textual query.
%
\item 
We instantiate the proposed query-aware dynamic attention by incorporating it in the Swin-Transformer and designing a flexible visual grounding framework \NetworkName\ based on the improved visual backbone.
\item 
%
We demonstrate that the proposed visual grounding method achieves significantly better performance than existing methods on five widely used public datasets.
%
\end{itemize}



==> 1.intro_backup_20211113.tex <==


In recent years, visual grounding is becoming an integral component of Vision-Language frameworks. Given an image and a natural language query, it can localize the referent object by returning a bounding box. By modeling the semantic alignments across vision and language, visual grounding framework can benefit the downstream tasks such as visual question answering\cite{zhu2016visual7w,gan2017vqs,wang2020general}, visually-grounded language navigation\cite{anderson2018vision,vogel2010learning} and image captioning\cite{you2016image,anderson2018bottom,chen2020say}.
%\begin{figure}
%\centering
%\begin{subfigure}[h]{1\linewidth}
%    \includegraphics[width=1\linewidth]{title_1_cropped.pdf}
%\end{subfigure}\vspace{0.05\linewidth}
%\begin{subfigure}[h]{1\linewidth}
%    \includegraphics[width=1\linewidth]{title_2_cropped.pdf}
%\end{subfigure}
%\caption{Upper: a typical visual grounding framework that uses two individual backbones to extract visual and textual features and perform cross-modal interaction. Below: our textual information infused visual grounding framework. Before the interaction, it first extracts the textual feature as guidance and guides the visual feature extraction.}
%\end{figure}
\begin{figure}[ht]
\centering
\includegraphics[width=1\linewidth]{figs/title_3_cropped.pdf}
\caption{(a): a typical end-to-end visual grounding framework that uses two individual encoders to extract visual and textual features and perform cross-modal interaction. (b): our textual guidance infused visual grounding framework that leverage the textual feature as guidance and guides the visual feature extraction to extract a query-aware feature map.}
\label{fig:title}
\end{figure}

Most conventional methods for visual grounding rely on a vision backbone. Two-stage methods use an off-the-shelf detector (e.g. Faster R-CNN\cite{ren2015faster}) to extract the regions and region-level features. In contrast, one-stage methods use a pre-trained fully convolutional network(e.g. Darknet53\cite{redmon2018yolov3}, ResNet\cite{he2016deep}) to extract pixel-level feature maps.

%However, the vision backbone is query-agnostic, which leads to many irrelevant regions or visual signals being extracted. As shown in \Cref{fig:title}(a), the extracted feature has a bias towards the detection task, which is sensitive to all salient objects, and most of them are irrelevant to the input query. Besides, the extracted feature is suitable for the pretraining classification task, which ignores the attribute and relationship, hinders the multi-modal interaction and limits localization accuracy. Moreover, the pre-trained backbone tends to extract features with different scales at specific layers, which benefits the detection task. However, in visual grounding, we only need to detect one object corresponding to the query. Existing methods use the feature map from the last layer or a query-agnostic multi-scale fusion(e.g., feature pyramid network) whose scale may be inconsistent with the referent object or be noisy. We call these two kinds of weakness semantic inconsistency and scale inconsistency. %感觉还需要进一步讨论视觉预训练会关注图像中大多数的物体，且由于用分类任务训练，对特征的抽取被局限在类比上，与开放域的任意文本对齐很困难。
These backbones are pre-trained on a detection task that needs a model to localize all objects in an image and classify them into close-set categories. We notice the visual grounding differs from the pre-training task and introduce two inconsistencies: 1) As shown in \Cref{fig:title}(a), the backbones are sensitive to all areas that contain salient objects. However, the visual grounding requires the model to localize only one object referred to by the query. We call it spatial inconsistency. 2) Backbones only utilize static visual features of different visual concepts to perform close-set classification. However, queries in visual grounding include open-ended entities and descriptions of attributes and relationships. The features required by the localization are determined by the query sentence dynamically. We call it semantic inconsistency. Because these backbones are query-agnostic, even they can be trained end-to-end, these two inconsistencies can still not be solved.

Recently several works have explored building query-aware vision backbone. \citet{chen2021ref} propose a query-aware Non-Maximum Suppression to filter query-irrelevant proposals before feeding them into the grounding module. However, this module can only be integrated into two-stage methods. Moreover, it can not affect proposal generation and feature extraction, limiting its generalizability and performance. \citet{kamath2021mdetr} extend DETR and propose a modulated detector that can detect objects conditioned on a text query. However, simply appending the textual sequence into the visual sequence will significantly change the original feature space. Thus they use 1.3M text-image pairs with explicit alignment annotation to train MDETR from scratch instead of initializing from the pre-trained DETR. The training data requirement limits its application and transferability.
% We notice that the main barrier to infuse textual feature into the vision backbone is that the textual feature space is different from the visual feature space learned by pre-trained weights. Therefore, this paper explores:\textit{ could we infuse textual guidance into the vision backbone while keeping the feature space to extract the query-consistent feature?} %这几段可以加一些reference

This paper proposes a query-aware vision backbone that can be trained end-to-end and only requires fine-tuning with in-domain datasets like most visual grounding models. As shown in \Cref{fig:title}(b), we consider giving visual encoder textual guidance by adjusting its attention distribution to keep the visual feature space and extract a query-consistent feature map. The high-quality feature map benefits the cross-modal alignment between the query and relevant region to make a correct prediction. To this end, we propose a novel asymmetric cross-modal interaction module called Query-aware Dynamic Attention to refine the visual feature map. The basic module does not simply fuse the visual and textual modality. Instead, it builds linear layers whose parameters are computed from the query's textual features. The text-dependent layers are applied to the visual feature to produce spatial and channel visual attention maps to reduce spatial and semantic inconsistencies, respectively. Note that the refining process does not change the shape and feature space of the input visual feature. It is easy to extend to various pre-trained vision backbones, e.g.,ViT\cite{dosovitskiy2020image}, ResNet\cite{he2016deep}.

We extend Swin-Transformer to a modulated vision backbone by incorporating proposed Query-aware Dynamic Attention to refine its feature extraction and multiscale fusion process. And we followed the recently proposed TransVG\cite{deng2021transvg} to build a visual grounding framework. Experiments on various common used phrase grounding and referring expression grounding datasets demonstrate the significant performance gains of the proposed modules. And the complete pipeline achieves the state-of-the-art performance, significantly surpassing the previous best methods.%要不要加一句说可视化结果显示在细粒度多模态交互之前，backbone得到的特征就已经关注于文本指向的区域了。

Our contributions are as follows:
\begin{itemize}
\item We propose to mitigate the spatial and semantic inconsistent issues by leveraging textual features to guide the vision backbone to extract query-aware feature maps.
\item We propose a novel Query-aware Dynamic Attention to refine the visual feature maps through textual guidance and further extend Swin-Transformer to a modulated vision backbone by incorporating the proposed module to guide its feature extraction and multiscale fusion process.
\item We also apply the novel backbone to a popular visual grounding framework to validate its merits. The results of a series of experiments on five widely used visual grounding datasets show that our methods obviously outperforms the state-of-the-art methods.
\end{itemize}



==> 2.related_work_backup_20211117.tex <==
\subsection{Visual Grounding}
%
The visual grounding methods can be categorized into two-stage methods and one-stage methods.
%

%
\textbf{Two-stage methods} divide the visual grounding process into two steps: generation and ranking.
%
Specifically, a module such as selective search~\cite{uijlings2013selective}, Edge-box~\cite{zitnick2014edge}, Region Proposal Network, or pre-trained detector~\cite{girshick2014rich,girshick2015fast,ren2015faster} will generate proposals that contain objects.
%
%lies.
%
Then a multimodal ranking network will measure the similarity between the query sentence and proposals and select the best matching. Early works~\cite{rohrbach2016grounding,mao2016generation,hu2016natural} only considered sentence-region level similarity. \citet{yu2018mattnet} decomposed the query sentence and image into three modular components related to subject, location, and relationship to models fine-grained similarity. Several studies~\cite{bajaj2019g3raphground,yang2019dynamic,yang2020graph,mu2021disentangled} incorporated graph learning to better model cross-modal alignment. \citet{chen2021ref} proposed Ref-NMS to use the query feature to guide the Non-Maximum Suppression to increase the recall of critical objects.

\textbf{One-stage methods} extract visual feature maps that maintaining the spatial structure and perform cross-modal interaction at pixel-level. The fused feature maps are further used to predict bounding boxes. \citet{yang2019fast} used a darknet\cite{redmon2018yolov3} to extract feature maps and broadcast the query embedding to each spatial location. Several works~\cite{liao2020real,yang2020improving,ye2021one} regarded multimodal interaction as a multiple step reasoning process to better understand the input query. \citet{huang2021look} extracted landmark feature with the guidance of linguistic description. The recent work TransVG~\cite{deng2021transvg} incorporated DETR encoder to extract visual features and proposed a transformer-based visual grounding framework. \citet{kamath2021mdetr} modeled the visual grounding as a modulated detection task and proposed a novel framework MDETR derived from the DETR detector. 

The most similar work to ours is Ref-NMS~\cite{chen2021ref} and MDETR~\cite{kamath2021mdetr}. However, Ref-NMS~\cite{chen2021ref} can only be integrated into two-stage methods. Moreover, it can not affect proposal generation and feature extraction. MDETR~\cite{kamath2021mdetr} requires 1.3M text-image pairs with explicit alignment annotation to train from scratch instead of initializing from the pre-trained DETR. In contrast, our \ModelName\ can be trained end-to-end and does not need multimodal pretraining.

\subsection{Transformer based Visual Backbones}
\citet{dosovitskiy2021an} proposed to extract image features by applying a pure Transformer architecture on image patches. The method achieves excellent results compared to state-of-the-art convolutional networks. These transformer-based visual backbones are called Vision Transformer (ViT). \citet{pmlr-v139-touvron21a} introduced training strategies to train a data-efficient ViT. \citet{yuan2021tokens} proposed a Tokens-to-Token transformation to obtain a global representation and a deep-narrow structure to improve its efficiency. Some works~\cite{chu2021we,han2021transformer} modified the ViT architecture for better performance. \citet{liu2021Swin} presented a novel hierarchical ViT called Swin Transformer. It computes the representation with shifted windowing scheme to allow for cross-window connection. Due to the fixed window size, the architecture has linear computational complexity with respect to image size.

\subsection{Multimodal Interaction}
In early studies, multimodal systems used simple interaction methods such as concatenation, element-wise product or summation, and fed to multilayer perception to learn the interaction~\cite{zadeh2017tensor,baltruvsaitis2018multimodal}. \citet{fukui2016multimodal} introduced a compact bilinear pooling to learn a more complex interaction. \citet{arevalo2017gated} presented a gated unit that can learn to decide how modalities influence the activation. \citet{nguyen2018improved,nagrani2021attention} used the cross-attention mechanism to enable dense, bi-directional interactions between the visual and textual modalities. \citet{NIPS2017_6fab6e3a} introduced Conditional Batch Normalization at channel-level to modulate visual feature maps by a linguistic embedding. \citet{vaezi20mmtm} used squeeze and excitation operations to fuse the multimodal features and recalibrate the channel-wise visual features. Some of these methods\cite{zadeh2017tensor,baltruvsaitis2018multimodal,arevalo2017gated,vaezi20mmtm,NIPS2017_6fab6e3a} only perform interaction at channel-level. However, spatial-level information is important to some downstream tasks, e.g., visual grounding and visual commonsense reasoning. The other methods~\cite{fukui2016multimodal,nguyen2018improved,nagrani2021attention} maintain the spatial structure to perform interaction but have a high computational cost. Moreover, these methods lead to uncertain feature spaces after their interactions, which is harmful to plug into the pre-trained networks.

==> 3.method_backup_20211115.tex <==
% Method

% 1. Preliminary 介绍Visual grounding任务以及基于TransVG的典型做法

% 2. Motivation and Overview 介绍我们对backbone改进的motivation，以及backbone的overview。这里就说明我们是extend Swin-transformer
% 3. Query-aware Dynamic Attention 和原论文结构一致 只是改名
%   1. Dynamic Linear Layer
%   2. Channel and Spatial Attention
% 4. Modulated Swin-Transformer 介绍如何extend swin，说明我们是在特征抽取阶段和多尺度融合阶段引入attention解决语义和空间不一致性。
%   1. Query-aware Attention in Feature Extraction 介绍在每个stage阶段插入一个attention模块
%   2. Multiscale Feature Fusion 介绍使用attention加权和patch merge的方式聚合多尺度特征
\subsection{Preliminary}
%
Visual grounding task aims at grounding a query sentence onto a region of an image.
%
It can be formulated as: given an image $I$ and a query sentence $q$, the model needs to learn to predict a bounding box $\mathbf{b}=\{x,y,w,h\}$ which exactly contains the target object expressed by the sentence.
%

%
Before introducing our method,
we firstly present a typical end-to-end visual grounding architecture TransVG~\cite{deng2021transvg}.
%
%as an example.
%
Given an image and a query sentence, there is a linguistic backbone, typically a pre-trained BERT model, extracting a 1D feature sequence $\mathbf{T}\in \mathbb{R}^{D_l\times N_l}$.
%
There is also a visual backbone (\eg DETR Encoder\cite{carion2020end}) extracting a flattened visual feature sequence $\mathbf{V} \in \mathbb{R}^{D_v\times N_v}$.
%
Two projection layers map the visual and linguistic features into the same feature space $\mathbb{R}^{D}$.
%
The projected visual and linguistic features are denoted by $\mathbf{p}_v\in \mathbb{R}^{D\times N_v}$ and $\mathbf{p}_l\in \mathbb{R}^{D\times N_l}$.
%
Then $p_v$ and $p_l$ are concatenated by inserting a learnable embedding (i.e., a [REG] token) at the beginning of the concatenated sequence.
%
The joint sequence is formulated as:
\begin{equation}
\begin{aligned}
\boldsymbol{x}_{0}=[\mathbf{p}_{r}, \underbrace{\mathbf{p}_{v}^{1}, \mathbf{p}_{v}^{2}, \cdots, \mathbf{p}_{v}^{N_{v}}}_{\text {visual tokens } \boldsymbol{p}_{v}}, \underbrace{\mathbf{p}_{l}^{1}, \mathbf{p}_{l}^{2}, \cdots, \mathbf{p}_{l}^{N_{l}}}_{\text {linguistic tokens } \boldsymbol{p}_{l}}],
\end{aligned}
\end{equation}
where $p_r$ is the learnable embedding of [REG] token.
%
%
Next, a multi-layer visual-linguistic transformer is applied to perform intra- and inter-modal reasoning on the joint sequence.
%
Finally, a prediction head takes the output representation of the [REG] token to predict the bounding box coordinates $\mathbf{b}$.
%
The smooth L1 loss~\cite{girshick2015fast} and giou loss~\cite{rezatofighi2019generalized} are used to train the framework.
%
The training objective can be formulated as:
\begin{equation}
\begin{aligned}
\mathcal{L}=\mathcal{L}_{smooth-l1}{(\mathbf{b},\mathbf{\hat{b}})}+\mathcal{L}_{giou}{(\mathbf{b},\mathbf{\hat{b}})},
\end{aligned}
\end{equation}
where $\mathbf{\hat{b}}$ is the ground-truth box.
%

% \begin{figure}[tb]
% \includegraphics[width=1\linewidth]{figs/overview_cropped.pdf}
% \caption{An overview of the \ModelName. (1) The language model first extract textual feature sequence. (2) Our query-aware vision backbone extracts and fuse multiscale visual features with textual guidance. (3) The visual and textual feature sequences are fed into a transformer, and a [REG] token representation is used to regress the bounding box.}
% \label{fig:model}
% \end{figure}
\begin{figure*}[tb]
\includegraphics[width=1\textwidth]{figs/overview_2_cropped.pdf}
\caption{(a) The typical visual grounding framework we used in this paper. (b) An overview of our \ModelName. The image is }
%\caption{An overview of the \ModelName. (1) The language model first extract textual feature sequence. (2) Our query-aware vision backbone extracts and fuse multiscale visual features with textual guidance. (3) The visual and textual feature sequences are fed into a transformer, and a [REG] token representation is used to regress the bounding box.}
\label{fig:model}
\end{figure*}
% 介绍一下visual grounding的三个组件 提出vision backbone的两个问题semantic inconsistency and scale inconsistency
% 解决方法是使用linguistic feature guide visual feature extraction in vision backbone
% 讲一下介绍顺序 首先介绍我们引入的新颖的查询驱动的attention模块 再介绍如何基于此方法构建一个Modulated and Multiscale Swin-Transformer 以解决这两个问题
\subsection{Motivation and Overview}
% 这里要说明motivation和intro对应
% 还有就是这里是介绍我们的swin的输入 中间架构 输出 要和后文描述贴合
% 正如之前所说明的，典型的visual grounding模型的vision backbone抽出的图像特征具有两种不一致 这阻碍了多模态交互，损害了模型的性能。
% 本文我们提出通过
\paragraph{Motivation}
As explained earlier, the visual features extracted from query-agnostic visual backbones have spatial and semantic inconsistencies. The inconsistencies hinder the multimodal interaction and hurt the models' performance.

In this paper, we propose to mitigate the spatial and semantic inconsistent issues by leveraging textual features to guide the visual backbone with Query-aware Dynamic Attention, which dynamically computes textual-dependent visual attention maps at spatial and channel level. We refine the feature maps during the feature extraction and multiscale fusion processes and output a query-consistent visual feature. We designing a flexible visual grounding framework based on the TransVG\footnote{https://github.com/djiajunustc/TransVG} by replacing the visual backbone with our \ModelName. The complete framework is shown in \Cref{fig:model} (a). We next focus on the visual backbone proposed in this paper.
\paragraph{Overview}
% 1. 大致介绍模型的结构
% 2. 我们下文的叙事顺序 xxx in Sec.x
We build the modulated multiscale visual backbone on a hierarchical visual backbone Swin-Transformer. We show the overall architecture in \Cref{fig:model} (b). During the feature extraction, a patch merge downsamples the input image and divides it into patches, and then there are four cascading stages. For simple representation, we denote the modules from pre-trained Swin-Transformer in the stage as Swin-Transformer Modules. Each stage also contains a Query-aware Dynamic Attention which takes the textual representation to refine the visual feature maps. Except for the first stage, the other three stages will obtain the feature of resolution divided by 2. During the multi-scale fusion stage, we fuse the features from each scale with the help of Query-aware Dynamic Attention and pooling operation. We flatten and concatenate the low-resolution features as the output token sequence of the backbone.

In the following, we first introduce the Query-aware Dynamic Attention (in \Cref{sec:QDA}) and how we build a modulated multiscale visual backbone with the Query-aware Dynamic Attention (in \Cref{sec:MMSwin}).
%The structure of TransVG is elegant and representative of most visual grounding frameworks. We notice a widespread problem that not all visual signals in images are helpful for the grounding task. However, the vision backbone pre-trained on detection tasks tends to extract all objects it has learned. Moreover, the backbone is trained to extract features for classification and is not enough for cross-modal alignment. There is also a problem that the cross-modal interaction module takes the feature map from the last layer or a query-agnostic multi-scale fusion whose scale may be inconsistent with the referent object or be noisy.

%To deal with these problems, we propose infusing the linguistic embedding into the vision backbone to guide the feature extraction and multi-scale feature fusion. To utilize the multi-scale feature, we first discard the vision backbone of TransVG because it only produces single-scale features. Instead, we use Swin-Transformer to extract multi-scale features. Then we introduce a novel Query-Driven Attention Mechanism, which leverages the linguistic embedding to drive the visual feature refinement. We further integrated the mechanism within the Swin-Transformer to guide the hierarchical feature extraction and multi-scale fusion. The improved backbone is called Modulated and Multiscale Swin-Transformer. We will cover the details in the following sections.
% \subsection{Query-Driven Attention Mechanism}
\subsection{Query-aware Dynamic Attention}
\label{sec:QDA}
In this section, we describe the details of our Query-aware Dynamic Attention (shown in \cref{fig:model}(c)). We first introduce the dynamic linear layer, which learns a linear transformation applied to the visual features. The difference is that the parameters of the linear transformation is not static and will be generated dynamically by textual features. We use dynamic linear layers to extract query-aware visual clues from the input visual features. We further introduce channel and spatial attention to refine the visual features with help of visual clues to produce query-consistent visual features.
\paragraph{Dynamic Linear Layer}
% \subsubsection{Query Guidance Function}
The existing visual feature extractor uses modules with static parameters to compute the visual feature maps. Feeding in the same image will output the same feature maps. However, in visual grounding, the textual features reveals the intention of the query. We present a dynamic linear which leverages the contextual textual feature $\mathbf{p}_l^c$ to guide the linear transformation to map an input vector $\mathbf{z}_{in}\in \mathbb{R}^{D^{in}}$ to $\mathbf{z}_{out}\in \mathbb{R}^{D^{out}}$. The dynamic linear layer can be formalized as follow:
\begin{equation}
\begin{aligned}
\mathbf{z}_{out}&=\mathrm{DyLinear}_{\mathcal{M}_l}(\mathbf{z}_{in})=\mathbf{W}_l^\intercal \mathbf{z}_{in}+\mathbf{b}_l
\end{aligned}
\end{equation}
where $\mathcal{M}_l=\{\mathbf{W}_l,\mathbf{b}_l\},\,\mathbf{W}_l\in \mathbb{R}^{D^{in}\times D^{out}},\, \mathbf{b}_l\in \mathbb{R}^{D^{out}}$, and $D^{in}$ and $D^{out}$ are the dimensions of input and output respectively.

We use a plain linear layer to generate the $\mathcal{M}_l$. The generator is denoted by $\mathcal{M}_l=\Psi(\mathbf{p}_l^c)$, where $\mathcal{M}^{'}_l\in\mathbb{R}^{(D^{in}+1)\ast D^{out}}$. In detail, we obtain a vector with shape $(D^{in}+1)*D^{out}$ and reshape it to $\mathcal{M}_l$. However, it is easy to find that the number of parameters in the generator is $D_l\ast ((D^{in}+1)\ast D^{out})$. We find that such large-scale parameters will slow down the training speed of the network and make it easier to be overfitting. Inspired by matrix factorization, we consider decomposing the $\mathcal{M}_l$ into two factor $\mathbf{U}\in \mathbb{R}^{(D^{in}+1)\times K}$ and $\mathbf{S}\in \mathbb{R}^{K\times D^{out}}$, where $\mathbf{U}$ is a matrix generate from $\mathbf{p}_l^c$, $\mathbf{S}$ is a static learnable matrix, $K$ is a hyper-parameter denote the factor dimension. The factor generator $\{\mathbf{W}_l,\mathbf{b}_l\}=\Psi^*(\mathbf{p}_l^c)$ can be formulated as follow:
\begin{equation}
\begin{aligned}
\mathbf{U}&=\mathrm{Reshape}({\mathbf{W}_{g}}^\intercal \mathbf{p}_l^c+\mathbf{b}_{g})
\end{aligned}
\end{equation}
where $\mathbf{W}_{g}\in \mathbb{R}^{D_l\times (D^{in}+1)\ast K}$ and $ \mathbf{b}_{g}\in \mathbb{R}^{(D^{in}+1)\ast K}$ are the parameters of the factor generator.% We first calculate the vector $U^{'}\in \mathbb{R}^{(D^{in}+1)\ast K}$ by the generator and further reshape it into a matrix $U\in \mathbb{R}^{(D^{in}+1)\times K}$.
\begin{equation}
\begin{aligned}
\mathcal{M}_l&=\mathbf{U}\mathbf{S}\\
\{\mathbf{W}_l,\mathbf{b}_l\} &= \mathrm{Split}(\mathcal{M}_l)\\
\end{aligned}
\end{equation}
Then the parameter matrix of dynamic linear layer $\mathcal{M}_l$ can be reconstructed by multiply $\mathbf{U}$ and $\mathbf{S}$. The $\mathbf{W}_l$ and $\mathbf{b}_l$ can be split from the matrix $\mathcal{M}_l$ along the first dimension. Finally, we reformulate the guidance function as follow:
\begin{equation}
\begin{aligned}
\mathbf{z}_{out}&=\mathrm{DyLinear}_{\mathcal{M}_l}(\mathbf{z}_{in})=\mathrm{DyLinear}_{\Psi^*(\mathbf{p}_l^c)}(\mathbf{z}_{in})
\end{aligned}
\end{equation}
%$p_l^c \in \mathbb{R}^{D_l},\, V\in \mathbb{R}^{K\times D^{out}},\, W^{dec}\in  \mathbb{R}^{D_l\times (D^{in}+1)\ast K},\, b^{dec}\in  \mathbb{R}^{(D^{in}+1)\ast K}$ backup the variable shape

Unless otherwise specified, the different $\mathrm{DyLinears}$ do not share parameters. And when the input is a multidimensional tensor, the layer transforms the input at the channel dimension.
%  如果不额外说明，dylinear之间不共享参数 如果输入的是一个多维tensor 默认对其channel维度进行特征变换
\paragraph{Channel and Spatial Attention}
% \subsubsection{Multi-level Feature Refinement}
% \begin{figure}[tb]
% \centering
% \includegraphics[width=1\linewidth]{figs/sc-attention_1_cropped.pdf}
% \caption{Diagram of the Query-aware Dynamic Attention}
% \label{fig:query_attention}
% \end{figure}

As we can obtain the visual clues, we consider refining the visual feature map by attention mechanism. As explained earlier, the pre-trained visual backbone is sensitive to all salient objects. Most of them are irrelevant to the query text. Therefore, The backbone only needs to attend to a few areas. Besides, The features useful for localization depend on the semantics contained in the query sentence (e.g. entities, descriptions of attributes and relationships). In other words, the importance of each channel in the features should change dynamically according to the query sentence. Inspired by the Convolutional Block Attention Module\cite{woo2018cbam}, we consider inferring a channel attention map $\mathbf{A}^{cl}$ to calibrate the semantic of feature for a better cross-modal alignment. And we further infer a spatial attention map $\mathbf{A}^{sl}$ from calibrated feature to reveal where the referent located.

Specifically, for a given visual feature $\mathbf{v}\in \mathbb{R}^{H\times W\times D_v}$, we first aggregate its spatial information by average pooling and maximum pooling and produce $\mathbf{v}^c_{max},\,\mathbf{v}^c_{mean}\in \mathbb{R}^{1\times 1\times D_v}$. We further build a dynamic multilayer perception consists of two dynamic linear layers. We use a ReLU activation after the first layer. The output dimension is the same as the input dimension. To reduce the number of parameter, we set the dimension of hidden states as $D_v/r$, where $r$ is the reduction ratio. By feeding the $\mathbf{v}^c_{max}$ and $\mathbf{v}^c_{mean}$ to the dynamic multilayer perception. We merge the two output features using summation. The channel attention map $\mathbf{A}^{cl}$ can be captured as follow:
\begin{equation}
\begin{aligned}
\mathbf{v}^{cl}_{mean}&=\mathrm{DyLinear}_1(\mathrm{ReLU}(\mathrm{DyLinear}_0(\mathbf{v}^c_{mean},p_l^c)),\mathbf{p}_l^c)\\
\mathbf{v}^{cl}_{max}&=\mathrm{DyLinear}_1(\mathrm{ReLU}(\mathrm{DyLinear}_0(\mathbf{v}^c_{max},p_l^c)),\mathbf{p}_l^c)\\
\mathbf{A}^{cl}&=\mathrm{sigmoid}(\mathbf{v}^{cl}_{mean}+\mathbf{v}^{cl}_{max})
\end{aligned}
\end{equation}


We perform element-wise multiplication between $\mathbf{v}$ and $\mathbf{A}^{cl}$ to form the representation of the channel refined visual feature, where the $A^{cl}$ are broadcast along the spatial dimension:
\begin{equation}
\begin{aligned}
\mathbf{V}^{'}&=\mathbf{A}^{cl}\otimes \mathbf{V}
\end{aligned}
\end{equation}

To generate a spatial attention map, instead pooling the channel dimension, we leverage another dynamic linear layer to reduce the channel dimension to learn areas interest to the query and apply a sigmoid function to generate the attention map. In short, The computing process is formulated as follow:
\begin{equation}
\begin{aligned}
\mathbf{A}^{sl}&=\mathrm{sigmoid}(\mathrm{DyLinear}_2(\mathbf{v}^{'},\mathbf{p}_l^c))\\
\mathbf{v}^{''}&=\mathbf{A}^{cl}\otimes \mathbf{v}^{'}
\end{aligned}
\end{equation}
where $\mathbf{A}^{sl}\in \mathbb{R}^{H\times W\times 1}$ is the spatial attention map and $\mathbf{v}^{''}$ is the spatial refined visual feature and also the output of our Query-aware Dynamic Attention.

\subsection{Query-modulated Transformer}
\label{sec:MMSwin}
In this section, we discuss how to use query-aware dynamic attention to extend Swin-Transformer\footnote{https://github.com/SwinTransformer/Swin-Transformer-Object-Detection} to a modulated visual backbone. %During feature extraction, we append a query-aware dynamic attention module at the end of each stage to refine the visual features generated by the swin-transformer blocks. Thanks to the hierarchical structure, we can obtain features at different scales from each stage. We introduce a Query-aware Multiscale Feature Fusion to fuse the hierarchical feature. We present the details below.

\paragraph{Query-aware Attention in Feature Extraction}
% \subsubsection{Modulated Swin-Transformer Block}
For a given image $I \in \mathbb{R}^{H\times W\times 3}$, a plain Swin-Transformer first embed $I$ to a $\mathbf{v}_0 \in \mathbb{R}^{\frac{H}{4}\times \frac{W}{4}\times 48}$. Then $\mathbf{v}_0$ is fed into four cascaded stages. Each stage $k$ receives the visual feature map $\mathbf{v}_{k-1}^*$ or $\mathbf{v}_0$ and generates a transformed feature map $\mathbf{v}_{k}$. We take the [CLS] representation of the input query sentence from BERT\cite{devlin2018bert} as the contextual query representation $\mathbf{p}_l^c$. We append a query-aware dynamic attention module at the end of each stage. It receives the transformed feature $\mathbf{v}_{k}$ from Swin-Transformer Blocks and produces a query-aware feature $\mathbf{v}_k^{*}$ to the next stage.
%  \begin{figure}[tb]
% \centering
% \includegraphics[width=1\linewidth]{figs/block_cropped.pdf}
% \caption{Modulated Multiscale Swin-Transformer Stage}
% \label{fig:stage}
% \end{figure}

\paragraph{Query-aware Attention in Multiscale Fusion}
% \subsubsection{Query-guided Multiscale Feature Fusion}
\label{sec:multiscale}
Thanks to the hierarchical structure, we can obtain features at different scales from each stage. Specifically, except the first stage, each stage reduce the resolution of feature map by a patch merging operator. In other words, the resolutions of the output of each stage are $\frac{H}{4}\times\frac{W}{4},\,\frac{H}{8}\times\frac{W}{8},\,\frac{H}{16}\times\frac{W}{16}$ and $\frac{H}{32}\times\frac{W}{32}$, respectively. Beside, the patch merging operator fuse the patch feature into channel which double the channel dimension. Thus the channel dimensions of the output of each stage are $C,\,2C,\,4C$ and $8C$.

Multiscale features are benefit to detect objects at different scale. however, because visual grounding require fine-grained interaction after visual backbone (\eg Cross Attention), high-resolution features will dramatically increase the computation. Previous works using the last feature or fuse the multiscale features by a query-agnostic fusion will obviously lose scale information or incorporate noise. As shown in \Cref{fig:model} (b), we propose to fuse the features with the \AttentionName. Specifically, we first use four $1\times 1$ convolutional layers to unify the channel dimensions to $D$. To filter out noisy signals in the feature maps, we build \AttentionName\ modules for the first three feature maps $\{\mathbf{v}^{*}_k |\,k=1,2,3 \}$. From $\mathbf{v}^{*}_0$, each module produce a weighted feature map with the same shape as before. We apply a $2\times 2$ mean pooling with stride=2 to reduce the resolution to be the same as next feature map $\mathbf{v}^{*}_k$ and compute the average of them to obtain $\mathbf{\bar{v}}^{*}_{k+1}$. Finally, the last feature map $\mathbf{\bar{v}}^{*}_{4}$ contains features interest to the query from all scales. To detect very large objects, we also apply a $2\times 2$ max pooling to obtain a $\frac{H}{64}\times\frac{W}{64}$ feature map $\mathbf{\bar{v}}^{*}_{5}$. We flatten and concatenate the $\mathbf{\bar{v}}^{*}_{4}$ and $\mathbf{\bar{v}}^{*}_{5}$ as the output token sequence $\mathbf{V}$.
%可以说相对于stage内部的，这里的Query-Driven Attention挖掘的是适合grounding的尺度的特征 同时去除不适合的尺度信息。(不过没有实验支撑 看着说吧)
% 这里一定要强调 这里的query attention...可以达到选择尺度的作用，因为如果某个尺度的信息不重要，模型可以将其尺度的attention map设为0以避免其信息向下传。而Swin Transforme中的模块需要为预训练权重服务，如果靠前的特征的权重很低，则只有few feature被传递到之后的模块，因此只有少量预训练权重发挥了作用，模型性能会急剧降低，因此我们需要引入额外的多尺度聚合模块。




==> 3.method_backup_20211116.tex <==
% Method

% 1. Preliminary 介绍Visual grounding任务以及基于TransVG的典型做法

% 2. Motivation and Overview 介绍我们对backbone改进的motivation，以及backbone的overview。这里就说明我们是extend Swin-transformer
% 3. Query-aware Dynamic Attention 和原论文结构一致 只是改名
%   1. Dynamic Linear Layer
%   2. Channel and Spatial Attention
% 4. Modulated Swin-Transformer 介绍如何extend swin，说明我们是在特征抽取阶段和多尺度融合阶段引入attention解决语义和空间不一致性。
%   1. Query-aware Attention in Feature Extraction 介绍在每个stage阶段插入一个attention模块
%   2. Multiscale Feature Fusion 介绍使用attention加权和patch merge的方式聚合多尺度特征
\subsection{Architecture}
%
{\color{red}In this section, we first formulate the visual grounding task and present the architecture of the framework we used.} Visual grounding task aims at grounding a query sentence onto a region of an image.
%
It can be formulated as: given an image $I$ and a query sentence $q$, the model needs to learn to predict a bounding box $\mathbf{b}=\{x,y,w,h\}$ which exactly contains the target object expressed by the sentence.
%

{\color{red}As shown in \Cref{fig:model} (a), our framework is based on a typical end-to-end visual grounding architecture TransVG~\cite{deng2021transvg}\footnote{https://github.com/djiajunustc/TransVG}}
%
%Before introducing our method,
%we firstly present a typical end-to-end visual grounding architecture TransVG~\cite{deng2021transvg}.
%
%as an example.
%
Given an image and a query sentence, there is a linguistic backbone, typically a pre-trained BERT model, extracting a 1D feature sequence $\mathbf{T}\in \mathbb{R}^{D_l\times N_l}$.
%
{\color{red}We propose the \NetworkName\ (described in \Cref{sec:network}) as a visual backbone to extract a flattened visual feature sequence $\mathbf{V} \in \mathbb{R}^{D_v\times N_v}$. The different is that the backbone take the contextual textual feature from the linguistic backbone to refine the feature extraction and multiscale fusion with the help of Query-aware Dynamic Attention\ (described in \Cref{sec:QDA}).}
%There is also a visual backbone ( ) extracting a flattened visual feature sequence $\mathbf{V} \in \mathbb{R}^{D_v\times N_v}$.
%
Two projection layers map the visual and linguistic features into the same feature space $\mathbb{R}^{D}$.
%
The projected visual and linguistic features are denoted by $\mathbf{p}_v\in \mathbb{R}^{D\times N_v}$ and $\mathbf{p}_l\in \mathbb{R}^{D\times N_l}$.
%
Then $\mathbf{p}_v$ and $\mathbf{p}_l$ are concatenated by inserting a learnable embedding (i.e., a [REG] token) at the beginning of the concatenated sequence.
%
The joint sequence is formulated as:
\begin{equation}
\begin{aligned}
\boldsymbol{X}=[\mathbf{p}_{r}, \underbrace{\mathbf{p}_{v}^{1}, \mathbf{p}_{v}^{2}, \cdots, \mathbf{p}_{v}^{N_{v}}}_{\text {visual tokens } \boldsymbol{p}_{v}}, \underbrace{\mathbf{p}_{l}^{c}, \mathbf{p}_{l}^{1}, \cdots, \mathbf{p}_{l}^{N_{l}}}_{\text {linguistic tokens } \boldsymbol{p}_{l}}],
\end{aligned}
\end{equation}
where $p_r$ is the learnable embedding of [REG] token.
%
%
Next, a multi-layer visual-linguistic transformer is applied to perform intra- and inter-modal reasoning on the joint sequence.
%
Finally, a prediction head takes the output representation of the [REG] token to predict the bounding box coordinates $\mathbf{b}$.
%
The smooth L1 loss~\cite{girshick2015fast} and giou loss~\cite{rezatofighi2019generalized} are used to train the framework.
%
The training objective can be formulated as:
\begin{equation}
\begin{aligned}
\mathcal{L}=\mathcal{L}_{smooth-l1}{(\mathbf{b},\mathbf{\hat{b}})}+\mathcal{L}_{giou}{(\mathbf{b},\mathbf{\hat{b}})},
\end{aligned}
\end{equation}
where $\mathbf{\hat{b}}$ is the ground-truth box.
%

% \begin{figure}[tb]
% \includegraphics[width=1\linewidth]{figs/overview_cropped.pdf}
% \caption{An overview of the \ModelName. (1) The language model first extract textual feature sequence. (2) Our query-aware vision backbone extracts and fuse multiscale visual features with textual guidance. (3) The visual and textual feature sequences are fed into a transformer, and a [REG] token representation is used to regress the bounding box.}
% \label{fig:model}
% \end{figure}
\begin{figure*}[tb]
\includegraphics[width=1\textwidth]{figs/overview_2_cropped.pdf}
\caption{(a) The QRNet-based visual grounding framework we used in this paper. (b) An overview of our \NetworkName. (c) The illustration of Query-aware Dynamic Attention.}
%\caption{An overview of the \ModelName. (1) The language model first extract textual feature sequence. (2) Our query-aware vision backbone extracts and fuse multiscale visual features with textual guidance. (3) The visual and textual feature sequences are fed into a transformer, and a [REG] token representation is used to regress the bounding box.}
\label{fig:model}
\end{figure*}
% 介绍一下visual grounding的三个组件 提出vision backbone的两个问题semantic inconsistency and scale inconsistency
% 解决方法是使用linguistic feature guide visual feature extraction in vision backbone
% 讲一下介绍顺序 首先介绍我们引入的新颖的查询驱动的attention模块 再介绍如何基于此方法构建一个Modulated and Multiscale Swin-Transformer 以解决这两个问题
\subsection{\NetworkName}
\label{sec:network}
% 这里要说明motivation和intro对应
% 还有就是这里是介绍我们的swin的输入 中间架构 输出 要和后文描述贴合
% 正如之前所说明的，典型的visual grounding模型的vision backbone抽出的图像特征具有两种不一致 这阻碍了多模态交互，损害了模型的性能。
% 本文我们提出通过
%\paragraph{Motivation}
%
{\color{red} In this section, we introduce our modulated visual backbone \NetworkName\ (\ModelName). An overview of the network is shown in \Cref{fig:model} (b).
The network consists of two phases: (1) Query-refined Feature Extraction extracts query-refined visual feature maps with a hierarchical structure. (2) Multi-scale Fusion fuses the maps at different scales with the guidance of the query feature. The two phases both rely on a novel Query-aware Dynamic Attention (\AttentionName), which dynamically computes textual-dependent visual attentions at spatial and channel level, to enable to compute features with query guidance.

Thus, in the following, we will first introduce implementation of the Query-aware Dynamic Attention. Then we detail the Query-refined Feature Extraction and Multi-scale Fusion.
}
%As illustrated in the introduction, the visual features extracted from conventional visual backbones always have the inconsistency issue,
%which hinders the effectiveness of the multimodal interaction and hurts the model performance.
%
%In this paper, we , which dynamically computes textual-dependent visual attentions at spatial and channel level.
%
%We instantiate the proposed Query-aware Dynamic Attention mechanism under a visual grounding framework similar as TransVG,
%
%where we adopt a new Query-modulated Transformer as an improved visual backbone.
%
%by replacing the visual backbone of the 
%The Query-modulated Transformer is designed based on Swin-Transformer to obtain query-consistent visual features by refining the feature maps with query-aware dynamic spatial and channel attentions.
%
%The attentions are dynamically computed based on textual features of the query to guide the learning of the visual backbone.
%

%
%with Query-aware Dynamic Attention, which dynamically computes textual-dependent visual attentions at spatial and channel level.
%
%instantiate the proposed Query-aware Dynamic Attention mechanism

%build a flexible visual grounding framework based on 
%to instantiate the proposed Query-aware Dynamic Attention 
%.
%
%
%, we propose to mitigate the inconsistency by leveraging textual features to guide the visual backbone with Query-aware Dynamic Attention, which dynamically computes textual-dependent visual attentions at spatial and channel level.
%
%We design a Query-modulated Transformer based on Swin-Transformer to instantiate the proposed Query-aware Dynamic Attention mechanism, which can obtain query-consistent visual features by refining the feature maps with attentions.
%
%during the feature extraction and multiscale fusion.
%

%
%We next focus on the proposed visual backbone of Query-modulated  Transformer.
%
%proposed in this paper.
%




%
%In the following, we will introduce more details of the Query-aware Dynamic Attention (in \Cref{sec:QDA}) and the improved visual backbone of Query-modulated Transformer (in \Cref{sec:MMSwin}).
%
%The structure of TransVG is elegant and representative of most visual grounding frameworks. We notice a widespread problem that not all visual signals in images are helpful for the grounding task. However, the vision backbone pre-trained on detection tasks tends to extract all objects it has learned. Moreover, the backbone is trained to extract features for classification and is not enough for cross-modal alignment. There is also a problem that the cross-modal interaction module takes the feature map from the last layer or a query-agnostic multi-scale fusion whose scale may be inconsistent with the referent object or be noisy.

%To deal with these problems, we propose infusing the linguistic embedding into the vision backbone to guide the feature extraction and multi-scale feature fusion. To utilize the multi-scale feature, we first discard the vision backbone of TransVG because it only produces single-scale features. Instead, we use Swin-Transformer to extract multi-scale features. Then we introduce a novel Query-Driven Attention Mechanism, which leverages the linguistic embedding to drive the visual feature refinement. We further integrated the mechanism within the Swin-Transformer to guide the hierarchical feature extraction and multi-scale fusion. The improved backbone is called Modulated and Multiscale Swin-Transformer. We will cover the details in the following sections.
% \subsection{Query-Driven Attention Mechanism}
\subsubsection{Query-aware Dynamic Attention}
\label{sec:QDA}
%
In this section, we describe the details of our Query-aware Dynamic Attention (shown in \cref{fig:model}(c)).
%
We first introduce the dynamic linear layer, which learns a linear transformation that can be applied on the visual features to compute the query-aware attentions.
%
Different from the conventional trainable linear layer,
the parameters of the dynamic linear layer are generated dynamically based on textual features.
%
%We use dynamic linear layers to extract query-aware visual clues from the input visual features.
%
Next, we will illustrate how to use the dynamic linear layer to compute query-aware channel and spatial attentions and obtain the query-consistent visual features. A pseudo-code is presented in the Appendix for better comprehension.
%
%refine the visual features with help of visual clues to produce .
%
\paragraph{Dynamic Linear Layer}
% Ye: 这部分怎么写能体现通用性 可插拔性 避免读者误以为z是我们模型的一部分？还没想好怎么写
% \subsubsection{Query Guidance Function}
%
Existing visual backbones use modules with static parameters to compute the visual feature maps,
%
where feeding in the same image will output the same feature maps.
%
However, in visual grounding, different queries for a single image may reveal different semantic information and intentions, which require different visual features.
%
We present a dynamic linear layer which can leverage the {\color{red}contextual textual feature $\mathbf{p}_l^c\in \mathbb{R}^{D_l}$}
%%%YXS:need to define the dimension
to guide the mapping from an given input vector $\mathbf{z}_{in}\in \mathbb{R}^{D^{in}}$ to the output $\mathbf{z}_{out}\in \mathbb{R}^{D^{out}}$.
%
The dynamic linear layer is formalized as follow:
\begin{equation}
\begin{aligned}
\mathbf{z}_{out}&=\mathrm{DyLinear}_{\mathcal{M}_l}(\mathbf{z}_{in})=\mathbf{W}_l^\intercal \mathbf{z}_{in}+\mathbf{b}_l
\end{aligned}
\end{equation}
where $\mathcal{M}_l=\{\mathbf{W}_l,\mathbf{b}_l\},\,\mathbf{W}_l\in \mathbb{R}^{D^{in}\times D^{out}},\, \mathbf{b}_l\in \mathbb{R}^{D^{out}}$.
%
$D^{in}$ and $D^{out}$ are the dimensions of input and output, respectively.


%
We use a plain linear layer to generate the $\mathcal{M}_l$.
%
The generator is denoted by $\mathcal{M}^{'}_l=\Psi(\mathbf{p}_l^c)$, where $\mathcal{M}^{'}_l\in\mathbb{R}^{(D^{in}+1)\ast D^{out}}$.
%
In detail, we predict a vector with shape $(D^{in}+1)*D^{out}$ which can be reshaped to $\mathcal{M}_l$.
%
However, it is easy to find that the number of parameters in the generator, i.e., {\color{red}$D_l\ast ((D^{in}+1)\ast D^{out})$}, is too large.
%%%YXS:the dimension D_l is not defined. 这个是文本序列的dimension 在overview有介绍 
%
Such large-scale parameters will slow down the training speed of the network and make it easier to be overfitting.
%
Inspired by matrix factorization, we consider decomposing the $\mathcal{M}_l$ into two factors $\mathbf{U}\in \mathbb{R}^{(D^{in}+1)\times K}$ and $\mathbf{S}\in \mathbb{R}^{K\times D^{out}}$, where $\mathbf{U}$ is a matrix generate from $\mathbf{p}_l^c$, $\mathbf{S}$ is a static learnable matrix, $K$ is a hyper-parameter denoting the factor dimension.
%
The factor generator $\{\mathbf{W}_l,\mathbf{b}_l\}=\Psi^*(\mathbf{p}_l^c)$ can be formulated as follow:
%\begin{equation}
%\begin{aligned}
%\end{aligned}
%\end{equation}
% We first calculate the vector $U^{'}\in \mathbb{R}^{(D^{in}+1)\ast K}$ by the generator and further reshape it into a matrix $U\in \mathbb{R}^{(D^{in}+1)\times K}$.
\begin{equation}
\begin{aligned}
& \mathbf{U}=\mathrm{Reshape}({\mathbf{W}_{g}}^\intercal \mathbf{p}_l^c+\mathbf{b}_{g}),\\
& \mathcal{M}_l=\mathbf{U}\mathbf{S},\\
& \{\mathbf{W}_l,\mathbf{b}_l\}= \mathrm{Split}(\mathcal{M}_l),\\
\end{aligned}
\end{equation}
where $\mathbf{W}_{g}\in \mathbb{R}^{D_l\times (D^{in}+1)\ast K}$ and $ \mathbf{b}_{g}\in \mathbb{R}^{(D^{in}+1)\ast K}$ are trainable parameters of the factor generator.
%
The parameter matrix $\mathcal{M}_l$ of the dynamic linear layer can be reconstructed by multiply $\mathbf{U}$ and $\mathbf{S}$.
%
The $\mathbf{W}_l$ and $\mathbf{b}_l$ can be split from the matrix $\mathcal{M}_l$ along the first dimension.
%
Finally, we reformulate the dynamic linear layer as follows:
\begin{equation}
\begin{aligned}
\mathbf{z}_{out}&=\mathrm{DyLinear}_{\mathcal{M}_l}(\mathbf{z}_{in})=\mathrm{DyLinear}_{\Psi^*(\mathbf{p}_l^c)}(\mathbf{z}_{in}).
\end{aligned}
\end{equation}
%$p_l^c \in \mathbb{R}^{D_l},\, V\in \mathbb{R}^{K\times D^{out}},\, W^{dec}\in  \mathbb{R}^{D_l\times (D^{in}+1)\ast K},\, b^{dec}\in  \mathbb{R}^{(D^{in}+1)\ast K}$ backup the variable shape

%
Unless otherwise specified, we use $\mathrm{DyLinear}(\mathbf{z}_{in})$ to represent a dynamic linear layer with $\mathbf{p}_l^c$ for simplify. And the different dynamic linear layers do not share parameters.
%
When the input is a multidimensional tensor, the dynamic linear layer transforms the input at the last dimension.

%%%YXS: channel表示tensor的哪个维度? 不能明确的话，channel dimension 改成 last dimension 是否可以？ 当时写的时候搜了一下channel dimension用得还挺多的，写成最后一个维度也可以
%
%  如果不额外说明，dylinear之间不共享参数 如果输入的是一个多维tensor 默认对其channel维度进行特征变换
\paragraph{Channel and Spatial Attention}
% \subsubsection{Multi-level Feature Refinement}
% \begin{figure}[tb]
% \centering
% \includegraphics[width=1\linewidth]{figs/sc-attention_1_cropped.pdf}
% \caption{Diagram of the Query-aware Dynamic Attention}
% \label{fig:query_attention}
% \end{figure}
%
%As we can obtain the visual clues, we consider refining the visual feature map by attention mechanism.
%
As explained in the introduction, the pre-trained visual backbone is sensitive to the objects defined in the pre-training task.
%
%that are contained in the training data.
%
However, most of these objects are irrelevant to the query text in visual grounding.
%
%Therefore, the backbone only needs to attend to a few areas.
%
Besides, the features useful for localization highly depend on the semantics contained in the query sentence (e.g. entities, descriptions of attributes and relationships).
%
In other words, the importance of each channel or each region of the feature map should change dynamically according to the query sentence.
%
Inspired by Convolutional Block Attention Module~\cite{woo2018cbam}, we consider inferring channel and spatial attentions, i.e., $\mathbf{A}^{cl}$ and $\mathbf{A}^{sl}$, along the separate  dimensions of the feature map to obtain adaptively refined features for a better cross-modal alignment.
%
%And we further infer a spatial attention map $\mathbf{A}^{sl}$ from calibrated feature to reveal where the referent located.
%

%
Specifically, for a given visual feature map $\mathbf{F}\in \mathbb{R}^{H\times W\times D_v}$, we first aggregate its spatial information by average pooling and maximum pooling and produce $\mathbf{F}^c_{max}\in \mathbb{R}^{1\times 1\times D_v},\mathbf{F}^c_{mean}\in \mathbb{R}^{1\times 1\times D_v}$.
%
Then, we build a dynamic multilayer perception consists of two dynamic linear layers.
%
We use a ReLU activation after the first layer.
%
The output dimension is the same as the input dimension.
%
To reduce the number of parameter, we set the dimension of hidden states as $D_v/r$, 
{\color{red}where $r=16$ is the reduction ratio.}
%%%YXS: r 作为超参数应该在实验中说明采用的值 
%%% Ye: 这里我直接用定值可以么
%
By feeding the $\mathbf{F}^c_{max}$ and $\mathbf{F}^c_{mean}$ to the dynamic multilayer perception, we merge the two output features using summation.
%
{\color{red}The channel attention map $\mathbf{A}^{cl}$} can be captured as follow:
%%%YXS:$\mathbf{A}^{cl}$的维度需要定义； 
{\color{red}
\begin{equation}
\begin{aligned}
\mathbf{F}^{cl}_{mean}&=\mathrm{DyLinear}_{1}(\mathrm{ReLU}(\mathrm{DyLinear}_{2}(\mathbf{F}^c_{mean}))\\
\mathbf{F}^{cl}_{max}&=\mathrm{DyLinear}_{1}(\mathrm{ReLU}(\mathrm{DyLinear}_{2}(\mathbf{F}^c_{max}))\\
\mathbf{A}^{cl}&=\mathrm{Sigmoid}(\mathbf{F}^{cl}_{mean}+\mathbf{F}^{cl}_{max}).
\end{aligned}
\end{equation}
}
%%%YXS:公式中的DyLinear0和DyLinear1的形式与前面的公式(5)的定义不匹配；
%%% Ye: 我在公式5之后给一个简化的符号表示

%
We perform element-wise multiplication between $\mathbf{F}$ and $\mathbf{A}^{cl}$ to form the channel-wise refined visual feature, where the $\mathbf{A}^{cl}$ is broadcast along the spatial dimension:
\begin{equation}
\begin{aligned}
\mathbf{F}^{'}&=\mathbf{A}^{cl}\otimes \mathbf{F}.
\end{aligned}
\end{equation}

%
To generate a spatial attention map, instead of pooling the channel dimension, we leverage another dynamic linear layer to reduce the channel dimension to learn areas of interest to the query and apply a Sigmoid function to generate the attention map.
%
In short, the computing process is formulated as follows:
\begin{equation}
\begin{aligned}
\mathbf{A}^{sl}&=\mathrm{Sigmoid}(\mathrm{DyLinear}_{3}(\mathbf{F}^{'}))\\
\mathbf{F}^{''}&=\mathbf{A}^{sl}\otimes \mathbf{F}^{'}
\end{aligned}
\end{equation}
where $\mathbf{A}^{sl}\in \mathbb{R}^{H\times W\times 1}$ is the spatial attention map and $\mathbf{F}^{''}$ is the spatially refined visual feature and also the output of our Query-aware Dynamic Attention.

\subsubsection{Query-refined Feature Extraction}
%
{\color{red}To extract query-aware feature maps, we extend the Swin-Transformer\footnote{https://github.com/SwinTransformer/Swin-Transformer-Object-Detection} to a modulated visual feature extractor.}
%In this section, we introduce how to use query-aware dynamic attention to extend a hierarchical Swin-Transformer\footnote{https://github.com/SwinTransformer/Swin-Transformer-Object-Detection} to a modulated visual backbone.
%
%During feature extraction, we append a query-aware dynamic attention module at the end of each stage to refine the visual features generated by the swin-transformer blocks. Thanks to the hierarchical structure, we can obtain features at different scales from each stage. We introduce a Query-aware Multiscale Feature Fusion to fuse the hierarchical feature. We present the details below.
%
%\paragraph{Overview}
% 1. 大致介绍模型的结构
% 2. 我们下文的叙事顺序 xxx in Sec.x
%
%Next, we introduce the overall architecture of the proposed Query-modulated Transformer, which is built based on a hierarchical Swin-Transformer.
%
As shown in \Cref{fig:model} (b),
%
%During the feature extraction, 
%a patch merging is first adopted to downsample 
%the input image is firstly downsampled and divided into patches by patch partition operation, and then there are four cascading stages.
%
%For simple representation, we denote the modules from pre-trained Swin-Transformer in the stage as Swin-Transformer Modules.
%
%Each stage contains modules from the corresponding stage of Swin-Transformer and a Query-aware Dynamic Attention module which takes the textual representation to compute the query-consistent visual feature maps.
%
%Except for the first stage, the other three stages divide the feature resolution by $2$.
%
%In the multi-scale fusion, we fuse the features obtained from different stages with the help of Query-aware Dynamic Attention mechanism and pooling operation.
%
%We flatten and concatenate the low-resolution features as the output token sequence of the backbone.
%
%\paragraph{Query-aware Attention in Feature Extraction.}
% \subsubsection{Modulated Swin-Transformer Block}
%
{\color{red}For a given image $I \in \mathbb{R}^{H\times W\times 3}$, 
a plain Swin-Transformer first embeds $I$ to $\mathbf{F}_0 \in \mathbb{R}^{\frac{H}{4}\times \frac{W}{4}\times 48}$ by a patch partition operation.
%
Then $\mathbf{F}_0$ is fed into four cascaded stages.
%
The $k$-th stage  receives the visual feature map $\mathbf{F}_{k-1}$ and generates a transformed feature map $\mathbf{F}_{k}$.
%
In this work, we take the [CLS] representation of the input query sentence from BERT~\cite{devlin2018bert} as the contextual query representation $\mathbf{p}_l^c$.
%
We append a query-aware dynamic attention module at the end of each stage.
%
It take the transformed feature $\mathbf{F}_{k}$ from Swin-Transformer blocks and produces a query-aware feature $\mathbf{F}_k^{*}$ to the next stage. Thus in the modulated Swin-Transformer, the last three stage receive the refined feature map $\mathbf{F}_{k-1}^{*}$ instead. The output of the query-refined feature extraction is a hierarchical feature list $[\mathbf{F}_{1}^{*},\mathbf{F}_{2}^{*},\mathbf{F}_{3}^{*},\mathbf{F}_{4}^{*}]$.}
%
%  \begin{figure}[tb]
% \centering
% \includegraphics[width=1\linewidth]{figs/block_cropped.pdf}
% \caption{Modulated Multiscale Swin-Transformer Stage}
% \label{fig:stage}
% \end{figure}

\subsubsection{Query-aware Multiscale Fusion.}\label{sec:multiscale}

% \subsubsection{Query-guided Multiscale Feature Fusion}
%
Multiscale features are benefit to detect objects at different scales~\cite{DBLP:conf/eccv/CaiFFV16}.
%
However, becuase visual grounding requires fine-grained interaction after visual backbone (\eg Cross Attention), high-resolution features will dramatically increase the computation.
%
Therefore, previous works always use the low-resolution features or fuse the multiscale features in a query-agnostic manner,
which will obviously lose scale information or incorporate noise.
%
Thanks to the hierarchical structure of the modulated Swin-Transformer, we can obtain multiscale features. We fuse the features obtained from different stages with the help of Query-aware Dynamic Attention mechanism and pooling operation.
%
We flatten and concatenate the low-resolution features as the output token sequence of the backbone.
%
Specifically, except the first stage, each stage reduces the resolution of feature map by a patch merging operator.
%
In other words, the resolutions of the output feature maps at four stages are $\frac{H}{4}\times\frac{W}{4},\,\frac{H}{8}\times\frac{W}{8},\,\frac{H}{16}\times\frac{W}{16}$ and $\frac{H}{32}\times\frac{W}{32}$, respectively.
%
Besides, the patch merging operator fuses the patch feature into the channel which doubles the channel dimension.
%
Thus the channel dimensions of the output at the four stages are $C,\,2C,\,4C$ and $8C$, respectively.
%
Next, we will introduce how to efficiently fuse these multiscale features with the guidance of the query text.
%


%
As shown in \Cref{fig:model} (b), we propose to fuse the output features at different stages with the help of \AttentionName.
%
Specifically, we first use four $1\times 1$ convolutional layers to unify the channel dimensions to $D$.
%
To filter out noisy signals in the feature maps, we build \AttentionName\ modules for the feature maps $\{\mathbf{F}^{*}_k |\,k=1,2,3 \}$ of the first three stages.
%
From {\color{red}$\mathbf{F}^{*}_k$}, the \AttentionName\ module produces a weighted feature map with the same size as the {\color{red}input}.
%
We apply a $2\times 2$ mean pooling with stride=2 to reduce the resolution to be the same as next feature map {\color{red}$\mathbf{F}^{*}_{k+1}$} and compute the average of them to obtain $\mathbf{\bar{F}}^{*}_{k+1}$.
%
Finally, the last feature map $\mathbf{\bar{F}}^{*}_{4}$ contains features of interest to the query from all scales.
%
To detect very large objects, we also apply a $2\times 2$ max pooling to obtain a $\frac{H}{64}\times\frac{W}{64}$ feature map $\mathbf{\bar{F}}^{*}_{5}$.
%
We flatten and concatenate the $\mathbf{\bar{F}}^{*}_{4}$ and $\mathbf{\bar{F}}^{*}_{5}$ as the output token sequence $\mathbf{V}$.
%
%可以说相对于stage内部的，这里的Query-Driven Attention挖掘的是适合grounding的尺度的特征 同时去除不适合的尺度信息。(不过没有实验支撑 看着说吧)
% 这里一定要强调 这里的query attention...可以达到选择尺度的作用，因为如果某个尺度的信息不重要，模型可以将其尺度的attention map设为0以避免其信息向下传。而Swin Transforme中的模块需要为预训练权重服务，如果靠前的特征的权重很低，则只有few feature被传递到之后的模块，因此只有少量预训练权重发挥了作用，模型性能会急剧降低，因此我们需要引入额外的多尺度聚合模块。




==> 4.experiment_backup_20211116.tex <==


\subsection{Datasets and Evaluation}%数据集看情况要不要扩展补充
We evaluate our method on phrase grounding dataset Flickr30K Entities\cite{plummer2015flickr30k} and referring expression grounding datasets RefCOCO\cite{yu2016modeling}, RefCOCO+\cite{yu2016modeling}, RefCOCOg\cite{mao2016generation} and ReferitGame\cite{kazemzadeh2014referitgame}. The details and statistics are summarized in Appendix. In phrase grounding the queries are phrases split from the captions and in referring expression grounding, they are referring expressions corresponding to the referred objects. We follow the same metric in \cite{deng2021transvg}. Specifically, a prediction is right if the IoU $>$ 0.5 between grounding-truth box and predicted bounding box.
% \begin{table}[ht]
% \centering
% \begin{tabular}{@{}llll@{}}
% \toprule
% Dataset            & Images & Instances & Queries  \\ \midrule
% RefCOCO            & 19,994 & 50,000    & 142,210 \\
% RefCOCO+           & 19,992 & 49,856    & 141,564 \\
% RefCOCOg           & 25,799 & 49,822    & 95,010  \\
% Flickr30K Entities & 31,783 & 427,000   & 427,000 \\
% ReferItGame        & 20,000 & 19,987    & 120,072 \\
% \bottomrule
% \end{tabular}
% \caption{Data statistics about RefCOCO, RefCOCO+, RefCOCOg, ReferItGame and  Flickr30K Entities dataset.}
% \label{tab:dataset_st}
% \end{table}


\subsection{Implementation Details}
The Swin-Transformer we extend is the Swin-S pre-trained with Mask-RCNN on MSCOCO~\cite{lin2014microsoft}\footnote{We excluded images in the validation and test split of the refcoco series from mscoco training set and retrained Swin-Transformer for fair comparison.}. We use $\mathrm{BERT}_{\mathrm{base}}$(uncased)\footnote{https://github.com/huggingface/pytorch-pretrained-BERT} for linguistic feature extraction. We set the intermediate dimension $D=256$ and the factor dimension $K=30$. We follow the TransVG~\cite{deng2021transvg} to process the input images and sentences. We also follow the training setting used in TransVG, which uses a AdamW optimizer with weight decay $10^{-4}$, sets the batch size to 64 and the dropout ratio to 0.1 for FFN in transformer. The learning rate of pre-trained parameters is set to $10^{-5}$ and the other is set to $10^{-4}$. The parameters without pre-training are randomly initialized with Xavier. We training our model for 160 epoches. The learning rate is multiplied by a factor of 0.1 at the epoch 60 for most dataset and 40 for Flickr30K Entities. We also follow the common used data augmentation strategies in ~\cite{liao2020real,yang2020improving,yang2019fast}.

\subsection{Quantitative Results}
We show the comparison results on ReferItGame and Flickr30k Entities in \Cref{tab:sub_main}. The ReferItGame collects queries by a cooperative game, requiring one player to write a referring expression for a specified object. The other one needs to click on the correct object. Queries in Flickr30k Entities are phrases in the caption. \ModelName\ also outperforms previous works. We replace the visual branch of TransVG with Swin-Transformer and denote it as TransVG(Swin) to explore the impact of replacing the backbone. The performance is similar to the origin TransVG, indicating that the accuracy gains are not from Swin-Transformer.
%这个表如果放backbone位置不够
\begin{table}[t]
\small
%\setlength{\tabcolsep}{1pt}
\centering

\begin{tabular}{@{}cccc@{}}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{Module}}               & \multicolumn{1}{c|}{\multirow{2}{*}{Backbone}} & \multicolumn{1}{c|}{ReferItGame}    & Flickr30K      \\
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{test}           & test           \\ \midrule
\multicolumn{4}{l}{\textbf{Two-stage}}                                                                                                                                      \\ \midrule
\multicolumn{1}{c|}{CMN~\cite{hu2017modeling}}              & \multicolumn{1}{c|}{VGG16}                     & \multicolumn{1}{c|}{28.33}          & -              \\
\multicolumn{1}{c|}{VC~\cite{zhang2018grounding}}           & \multicolumn{1}{c|}{VGG16}                     & \multicolumn{1}{c|}{31.13}          & -              \\
\multicolumn{1}{c|}{MAttNet~\cite{yu2018mattnet}}           & \multicolumn{1}{c|}{ResNet-101}                & \multicolumn{1}{c|}{29.04}          & -              \\
\multicolumn{1}{c|}{Similarity net~\cite{wang2018learning}} & \multicolumn{1}{c|}{ResNet-101}                & \multicolumn{1}{c|}{34.54}          & 50.89          \\
\multicolumn{1}{c|}{LCMCG~\cite{liu2020learning}}           & \multicolumn{1}{c|}{ResNet-101}                & \multicolumn{1}{c|}{-}              & 76.74          \\
\multicolumn{1}{c|}{DIGN~\cite{mu2021disentangled}}         & \multicolumn{1}{c|}{VGG-16}                    & \multicolumn{1}{c|}{{\ul 65.15}}    & {\ul 78.73}    \\ \midrule
\multicolumn{4}{l}{\textbf{One-stage}}                                                                                                                                      \\ \midrule
\multicolumn{1}{c|}{SSG~\cite{chen2018real}}                & \multicolumn{1}{c|}{DarkNet-53}                & \multicolumn{1}{c|}{54.24}          & -              \\
\multicolumn{1}{c|}{FAOA~\cite{yang2019fast}}               & \multicolumn{1}{c|}{DarkNet-53}                & \multicolumn{1}{c|}{60.67}          & 68.71          \\
\multicolumn{1}{c|}{RCCF~\cite{liao2020real}}               & \multicolumn{1}{c|}{DLA-34}                    & \multicolumn{1}{c|}{63.79}          & -              \\
\multicolumn{1}{c|}{ReSC-Large~\cite{yang2020improving}}    & \multicolumn{1}{c|}{DarkNet-53}                & \multicolumn{1}{c|}{64.60}          & 69.28          \\
\multicolumn{1}{c|}{SAFF~\cite{ye2021one}}                  & \multicolumn{1}{c|}{DarkNet-53}                & \multicolumn{1}{c|}{66.01}          & 70.71          \\
\multicolumn{1}{c|}{TransVG~\cite{deng2021transvg}}         & \multicolumn{1}{c|}{ResNet-101}                & \multicolumn{1}{c|}{70.73}          & {\ul 79.10}    \\
\multicolumn{1}{c|}{TransVG\,(Swin)}                       & \multicolumn{1}{c|}{Swin-S}                    & \multicolumn{1}{c|}{{\ul 70.86}}    & 78.18          \\ \midrule
\multicolumn{1}{c|}{\ModelName\ (ours)}                    & \multicolumn{1}{c|}{Swin-S}                    & \multicolumn{1}{c|}{\textbf{74.61}} & \textbf{81.95} \\ \bottomrule
\end{tabular}
\caption{The performance comparisons (Acc@0.5) on ReferItGame and Flickr30K Entities.}
\label{tab:sub_main}
\end{table}


\begin{table*}[ht]
\centering
\begin{tabular}{@{}ccccccccccc@{}}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{Models}}             & \multicolumn{1}{c|}{\multirow{2}{*}{Backbone}} & \multicolumn{3}{c|}{RefCOCO}                                          & \multicolumn{3}{c|}{RefCOCO+}                                         & \multicolumn{3}{c}{RefCOCOg}                     \\
\multicolumn{1}{c|}{}                                    & \multicolumn{1}{c|}{}                          & val            & testA          & \multicolumn{1}{c|}{testB}          & val            & testA          & \multicolumn{1}{c|}{testB}          & val-g          & val-u          & test-u         \\ \midrule
% \multicolumn{11}{l}{\textbf{Pre-training}}                                                                                                                                                                                                                                                                               \\ \midrule
% \multicolumn{1}{c|}{MDETR~\cite{kamath2021mdetr}}         & \multicolumn{1}{c|}{ResNet-101}                & 87.51          & 89.40          & \multicolumn{1}{c|}{81.41}          & 79.52          & 84.09          & \multicolumn{1}{c|}{70.09}          & -              & 83.35          & 80.89          \\ \midrule
\multicolumn{11}{l}{\textbf{Two-stage}}                                                                                                                                                                                                                                                                               \\ \midrule
\multicolumn{1}{c|}{CMN~\cite{hu2017modeling}}            & \multicolumn{1}{c|}{VGG16}                     & -              & 71.03          & \multicolumn{1}{c|}{65.77}          & -              & 54.32          & \multicolumn{1}{c|}{47.76}          & 57.47          & -              & -              \\
\multicolumn{1}{c|}{VC~\cite{zhang2018grounding}}         & \multicolumn{1}{c|}{VGG16}                     & -              & 73.33          & \multicolumn{1}{c|}{67.44}          & -              & 58.40          & \multicolumn{1}{c|}{53.18}          & 62.30          & -              & -              \\
\multicolumn{1}{c|}{MAttNet~\cite{yu2018mattnet}}         & \multicolumn{1}{c|}{ResNet-101}                & 76.65          & 81.14          & \multicolumn{1}{c|}{69.99}          & 65.33          & 71.62          & \multicolumn{1}{c|}{56.02}          & -              & 66.58          & 67.27          \\
\multicolumn{1}{c|}{Ref-NMS~\cite{chen2021ref}}           & \multicolumn{1}{c|}{ResNet-101}                & {\ul 78.82}    & 82.71          & \multicolumn{1}{c|}{{\ul 73.94}}    & 66.95          & 71.29          & \multicolumn{1}{c|}{{\ul 58.40}}    & -              & {\ul 68.89}    & {\ul 68.67}    \\
\multicolumn{1}{c|}{LGRANs~\cite{wang2019neighbourhood}}  & \multicolumn{1}{c|}{VGG16}                     & -              & 76.60          & \multicolumn{1}{c|}{66.40}          & -              & 64.00          & \multicolumn{1}{c|}{53.40}          & 61.78          & -              & -              \\
\multicolumn{1}{c|}{RvG-Tree~\cite{hong2019learning}}     & \multicolumn{1}{c|}{ResNet-101}                & 75.06          & 78.61          & \multicolumn{1}{c|}{69.85}          & 63.51          & 67.45          & \multicolumn{1}{c|}{56.66}          & -              & 66.95          & 66.51          \\
\multicolumn{1}{c|}{CM-Att-Erase~\cite{liu2019improving}} & \multicolumn{1}{c|}{ResNet-101}                & 78.35          & {\ul 83.14}    & \multicolumn{1}{c|}{71.32}          & {\ul 68.09}    & {\ul 73.65}    & \multicolumn{1}{c|}{58.03}          & {\ul 68.67}    & -              & -              \\
\multicolumn{1}{c|}{NMTree~\cite{liu2019learning}}        & \multicolumn{1}{c|}{ResNet-101}                & 76.41          & 81.21          & \multicolumn{1}{c|}{70.09}          & 66.46          & 72.02          & \multicolumn{1}{c|}{57.52}          & 64.62          & 65.87          & 66.44          \\ \midrule
\multicolumn{11}{l}{\textbf{One-stage}}                                                                                                                                                                                                                                                                               \\ \midrule
\multicolumn{1}{c|}{SSG~\cite{chen2018real}}              & \multicolumn{1}{c|}{DarkNet-53}                & -              & 76.51          & \multicolumn{1}{c|}{67.50}          & -              & 62.14          & \multicolumn{1}{c|}{49.27}          & 47.47          & 58.80          & -              \\
\multicolumn{1}{c|}{FAOA~\cite{yang2019fast}}             & \multicolumn{1}{c|}{DarkNet-53}                & 72.54          & 74.35          & \multicolumn{1}{c|}{68.50}          & 56.81          & 60.23          & \multicolumn{1}{c|}{49.60}          & 56.12          & 61.33          & 60.36          \\
\multicolumn{1}{c|}{RCCF~\cite{liao2020real}}             & \multicolumn{1}{c|}{DLA-34}                    & -              & 81.06          & \multicolumn{1}{c|}{71.85}          & -              & 70.35          & \multicolumn{1}{c|}{56.32}          & -              & -              & 65.73          \\
\multicolumn{1}{c|}{ReSC-Large~\cite{yang2020improving}}  & \multicolumn{1}{c|}{DarkNet-53}                & 77.63          & 80.45          & \multicolumn{1}{c|}{72.30}          & 63.59          & 68.36          & \multicolumn{1}{c|}{56.81}          & 63.12          & 67.30          & 67.20          \\
\multicolumn{1}{c|}{SAFF~\cite{ye2021one}}                & \multicolumn{1}{c|}{DarkNet-53}                & 79.26          & 81.09          & \multicolumn{1}{c|}{76.55}          & 64.43          & 68.46          & \multicolumn{1}{c|}{58.43}          & -              & 68.94          & 68.91          \\
\multicolumn{1}{c|}{HFRN~\cite{qiu2020language}}          & \multicolumn{1}{c|}{ResNet-101}                & 79.76          & {\ul 83.12}    & \multicolumn{1}{c|}{75.51}          & 66.80          & 72.53          & \multicolumn{1}{c|}{59.09}          & -              & {\ul 69.71}    & 69.08          \\
\multicolumn{1}{c|}{ISRL~\cite{sun2021iterative}}         & \multicolumn{1}{c|}{ResNet-101}                & -              & 74.27          & \multicolumn{1}{c|}{68.10}          & -              & 71.05          & \multicolumn{1}{c|}{58.25}          & -              & -              & {\ul 70.05}    \\
\multicolumn{1}{c|}{LBYL-Net~\cite{huang2021look}}        & \multicolumn{1}{c|}{DarkNet-53}                & 79.67          & 82.91          & \multicolumn{1}{c|}{74.15}          & {\ul 68.64}    & {\ul 73.38}    & \multicolumn{1}{c|}{{\ul 59.49}}    & 62.70          & -              & -              \\
\multicolumn{1}{c|}{TransVG~\cite{deng2021transvg}}       & \multicolumn{1}{c|}{ResNet-101}                & {\ul 81.02}    & 82.72          & \multicolumn{1}{c|}{{\ul 78.35}}    & 64.82          & 70.70          & \multicolumn{1}{c|}{56.94}          & {\ul 67.02}    & 68.67          & 67.73          \\ \midrule
\multicolumn{1}{c|}{\ModelName\ (ours)}                  & \multicolumn{1}{c|}{Swin-S}                    & \textbf{84.01} & \textbf{85.85} & \multicolumn{1}{c|}{\textbf{82.34}} & \textbf{72.94} & \textbf{76.17} & \multicolumn{1}{c|}{\textbf{63.81}} & \textbf{74.05} & \textbf{75.80} & \textbf{75.52} \\ \bottomrule
\end{tabular}
\caption{The performance comparisons (Acc@0.5) on ReferCOCO, ReferCOCO+,ReferCOCOg. The previous best two-stage and one-stage performances are highlighted with underline, respectively. We highlight our results in bold. The results demonstrate our method outperforms all state-of-the-art one-stage and two-stage methods.}
\label{tab:main}
\end{table*}

We also present the accuracy comparison with state-of-the-art methods on ReferCOCO, ReferCOCO+ and ReferCOCOg in \Cref{tab:main}. In ReferCOCO and ReferCOCO+ datasets, referred objects are people in ``testA" and could be common objects in ``testB". The expressions in ReferCOCOg are much longer than in other datasets. Note that TransVG uses a ResNet-101 and a DETR encoder split from a pre-trained DETR framework. The visual backbone is more powerful than other ResNet-101. Because the MDETR\cite{kamath2021mdetr} uses large-scale image-caption pairs with bounding box annotations for pre-training, the other methods only use the corresponding train split when evaluated on each dataset. For fair, we do not present its performances.


We observe that our \ModelName\ greatly outperforms all two-stage and one-stage stage-of-the-art methods. In RefCOCO and RefCOCO+ datasets, our method gains 2.37\%$\sim$2.79\% absolute improvement in ``testA" and 3.99\%$\sim$4.32\% in ``testB". When the referred objects are arbitrary, the inconsistent issue will be more obvious, and our modulated backbone can better filter irrelevant objects and correct the representation with textual guidance. In the RefCOCOg test split, we notice that ISRL~\cite{sun2021iterative} performs better than TransVG~\cite{deng2021transvg}. It models the visual grounding to a Markov decision process that handles long expressions iterative by filtering out irrelevant areas. However, the limited action space makes it easy to converge to a local optimum. Our model does not modify the Visual-Linguistic Transformer in the TransVG but only provides query-consistent visual features. The performance is greatly improved which proves that our query-aware refinement is more effective to model the multimodal representation for visual grounding.

\subsection{Ablation Study}

\begin{table}[tb]
\small
\setlength{\tabcolsep}{8pt}
\centering
\begin{tabular}{c|cc|cc}
\toprule
\multirow{2}{*}{Models} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Feature \\ Extraction\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Multiscale\\ Fusion\end{tabular}} & \multicolumn{2}{l}{ReferItGame} \\
 &  &  & val & test \\
 \midrule
\ModelName & \CheckmarkBold & \CheckmarkBold  & \bf 76.84 & \bf 74.61 \\
\midrule
(a) & \CheckmarkBold & \XSolidBrush & 74.31 & 72.09 \\
(b) & \XSolidBrush & \CheckmarkBold & 73.63 & 71.39 \\
(c) & \XSolidBrush & \XSolidBrush   & 73.25  & 70.86 \\ 
 \bottomrule
\end{tabular}
\caption{The ablations of the proposed two modules.} \label{tab:abl_module}
\vspace{1.5em}
\begin{tabular}{c|cc|cc}
\toprule
\multirow{2}{*}{Models} & \multirow{2}{*}{\tabincell{c}{Channel\\ Attention}} & \multirow{2}{*}{\tabincell{c}{Spatial\\ Attention}} & \multicolumn{2}{c}{ReferItGame} \\
 &  &  & val & test \\
 \midrule
\ModelName & \CheckmarkBold & \CheckmarkBold  & \bf 76.84 & \bf 74.61 \\
\midrule
(d) & \CheckmarkBold & \XSolidBrush & 74.35 & 72.02 \\
(e) & \XSolidBrush & \CheckmarkBold & 74.41 & 71.80 \\
 \bottomrule
\end{tabular}
\caption{The ablations of the query-driven attention.}
\label{tab:abl_attention}
\end{table}

We conduct several ablation studies on ReferItGame to reveal the effectiveness of our proposed modules.


We first study the effectiveness of the two proposed modules. As shown in \Cref{tab:abl_module}, when only adopting \AttentionName\ during feature extraction, the performance is improved by 1.06\% in ``val" and 1.27\% in ``test", respectively. When only adopting \AttentionName\ during multiscale fusion, the performance is improved by 0.38\% and 0.53\%. When enhancing both two processes, the performance is improved by 3.63\% and 3.59\%. We find that when the feature extraction is not modified, the features of each scale are still query-inconsistent. {\color{red}It is hard for the fusion module to learn both feature refinement and query-aware multiscale fusion from scratch without the help of pre-training knowledge.} Thus there is still much noise in the fused multiscale features, which limits its improvement. When the feature extraction is query-aware, the multiscale fusion can significantly improve the model's performance.

We further study the effectiveness of spatial attention and channel attention in the \AttentionName. Note that the settings affect both the feature extraction and multiscale fusion. Spatial attention can filter out irrelevant areas. And channel attention can redistribution the importance of the features to fit different query sentences. The results shown in the \Cref{tab:abl_attention} demonstrate that spatial and channel attention are both effective.

\begin{figure}[tb]
\centering
\includegraphics[width=\linewidth]{figs/factor.pdf}
\caption{The effect of factor dimension $K$.}
\label{fig:factor}
\end{figure}
We study the hyper-parameter $K$ which denotes the factor dimension. We report the accuracy of model with $K=\{10,30,50,70\}$ in \Cref{fig:factor}. When $K$ is small, the \AttentionName\ can not learn the transformation well. And when $K$ is large, the \AttentionName\ is easy to overfitting and perform worse on validation set. We take the best $K=30$ on validation set as our default setting.
\subsection{Qualitative Results}
\begin{figure}[tb]
\centering
\includegraphics[width=\linewidth]{figs/vis_1_cropped.pdf}
\caption{Visualization of activation maps from plain Swin-Transformer and the modulated backbone of our \ModelName\ . Green: grounding truth; blue: prediction of our model}
\label{fig:vis}
\end{figure}

We show the qualitative examples of our \ModelName\ framework on the RefCOCO dataset in \Cref{fig:vis}. The first row shows the activation maps from plain Swin-Transformer. The second row shows the activation maps from our modulated visual backbone.  We observe that query-agnostic Swin-Transformer tends to extract features of all salient objects. In comparison, our query-aware backbone can understand entities words, \eg, ``glass'', and appearance descriptions, \eg, ``light blue tall''. It also can perform reasoning through location words, \eg, ``upper left'' and ``nearest''. The produced activation maps are highly relevant to the query sentences.
% \begin{figure*}[htb]
% \centering
% \includegraphics[width=0.8\textwidth]{figs/vis_cropped.pdf}
% \caption{vis}
% \label{fig:model}
% \end{figure*}

==> InstructionCPVR.tex <==



%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of cvpr.sty to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the CVPR70 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.


% Update the cvpr.cls to do the following automatically.
% For this citation style, keep multiple citations in numerical (not
% chronological) order, so prefer \cite{Alpher03,Alpher02,Authors14} to
% \cite{Alpher02,Alpher03,Authors14}.


\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

%------------------------------------------------------------------------
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

%------------------------------------------------------------------------
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.


==> intro_bak.tex <==


In recent years, visual grounding is becoming an integral component of Vision-Language frameworks. Given an image and a natural language query, it can localize the referent object by returning a bounding box. By modeling the semantic alignments across vision and language, visual grounding framework can benefit the downstream tasks such as visual question answering\cite{zhu2016visual7w,gan2017vqs,wang2020general}, visually-grounded language navigation\cite{anderson2018vision,vogel2010learning} and image captioning\cite{you2016image,anderson2018bottom,chen2020say}.
%\begin{figure}
%\centering
%\begin{subfigure}[h]{1\linewidth}
%    \includegraphics[width=1\linewidth]{title_1_cropped.pdf}
%\end{subfigure}\vspace{0.05\linewidth}
%\begin{subfigure}[h]{1\linewidth}
%    \includegraphics[width=1\linewidth]{title_2_cropped.pdf}
%\end{subfigure}
%\caption{Upper: a typical visual grounding framework that uses two individual backbones to extract visual and textual features and perform cross-modal interaction. Below: our textual information infused visual grounding framework. Before the interaction, it first extracts the textual feature as guidance and guides the visual feature extraction.}
%\end{figure}
\begin{figure}[ht]
\centering
\includegraphics[width=1\linewidth]{figs/title_3_cropped.pdf}
\caption{(a): a typical end-to-end visual grounding framework that uses two individual encoders to extract visual and textual features and perform cross-modal interaction. (b): our textual guidance infused visual grounding framework that leverage the textual feature as guidance and guides the visual feature extraction to extract a query-aware feature map.}
\label{fig:title}
\end{figure}

Most conventional methods for visual grounding rely on a vision backbone. Two-stage methods use an off-the-shelf detector (e.g. Faster R-CNN\cite{ren2015faster}) to extract the regions and region-level features. In contrast, one-stage methods use a pre-trained fully convolutional network(e.g. Darknet53\cite{redmon2018yolov3}, ResNet\cite{he2016deep}) to extract pixel-level feature maps.

However, the vision backbone is query-agnostic, which leads to many irrelevant regions or visual signals being extracted. As shown in \Cref{fig:title}(a), the extracted feature has a bias towards the detection task, which is sensitive to all salient objects, and most of them are irrelevant to the input query. Besides, the extracted feature is suitable for the pretraining classification task, which ignores the attribute and relationship, hinders the multi-modal interaction and limits localization accuracy. Moreover, the pre-trained backbone tends to extract features with different scales at specific layers, which benefits the detection task. However, in visual grounding, we only need to detect one object corresponding to the query. Existing methods use the feature map from the last layer or a query-agnostic multi-scale fusion(e.g., feature pyramid network) whose scale may be inconsistent with the referent object or be noisy. We call these two kinds of weakness semantic inconsistency and scale inconsistency. %感觉还需要进一步讨论视觉预训练会关注图像中大多数的物体，且由于用分类任务训练，对特征的抽取被局限在类比上，与开放域的任意文本对齐很困难。



The key to overcoming these inconsistencies is to leverage the query text to guide feature extraction of the vision backbone network. Recently several works have explored some solutions. \citet{chen2021ref} propose a query-aware Non-Maximum Suppression to filter query-irrelevant proposals before feeding them into the grounding module. However, this module can only be integrated into two-stage methods and can not affect feature extraction, limiting its generalizability and performance. \citet{kamath2021mdetr} extend DETR and proposes a modulated detector that can detect objects conditioned on a text query. But the redesigned framework makes the pre-trained DETR weights unavailable, and it requires 1.3M text-image pairs with explicit alignment annotation for training. These weaknesses limit its application and transferability. We notice that the main barrier to infuse textual feature into the vision backbone is that the textual feature space is different from the visual feature space learned by pre-trained weights. Therefore, this paper explores:\textit{ could we infuse textual guidance into the vision backbone while keeping the feature space to extract the query-consistent feature?} %这几段可以加一些reference

In this paper, as shown in \Cref{fig:title}(b), instead of directly fusing the textual feature into the visual feature, we consider giving visual encoder textual guidance by adjusting its attention distribution with textual guidance to avoid semantic inconsistency and extract a query-aware feature map. The high-quality feature map benefits the cross-modal alignment between the query and relevant region to make a correct prediction. To this end, we propose a novel asymmetric cross-modal interaction mechanism called Query-Driven Attention Mechanism to produce text-guided visual attention maps. The basic mechanism does not simply fuse the visual and textual modality. Instead, it produces the textual feature parameters to obtain a text-dependent linear layer to better model the text-guided attention estimation. We further propose a Modulated Swin-Transformer Block that inherits pre-trained weights and leverages the textual guidance to refine visual features at spatial and channel levels. Note that the refining process does not change the shape and feature space of the input visual feature. It is easy to extend to other vision backbones, e.g.,ViT\cite{dosovitskiy2020image}, ResNet\cite{he2016deep}.

To avoid scale inconsistency, we propose the Query-guided Multiscale Feature Fusion to fuse the multiscale feature. We use a patch merging strategy to compress the feature of interest to the query from the high-resolution map. Furthermore, we investigate a bottom-up pathway to fuse the multiscale feature maps to low-scale feature maps with textual guidance.

We extend Swin-Transformer to a modulated vision backbone by incorporating proposed Modulated Swin-Transformer Block and Query-guided Multiscale Feature Fusion without a multi-modal pretraining. And we followed the recently proposed TransVG\cite{deng2021transvg} to build a visual grounding framework. Experiments on various common used phrase grounding and referring expression grounding datasets demonstrate the significant performance gains of the proposed modules. And the complete pipeline achieves the state-of-the-art performance, significantly surpassing the previous best methods.%要不要加一句说可视化结果显示在细粒度多模态交互之前，backbone得到的特征就已经关注于文本指向的区域了。

Our contributions are as follows:
\begin{itemize}
\item We propose to mitigate the semantic and scale inconsistent issues by infusing textual guidance into the vision backbone to extract query-aware feature maps.
\item We extend Swin-Transformer to a modulated vision backbone by incorporating the proposed Modulated Swin-Transformer Block and Query-guided Multiscale Feature Fusion. We also apply the novel backbone to a popular visual grounding framework to validate its merits.
\item We conduct a series of experiments on five widely used visual grounding datasets. The results show that our methods obviously outperforms the state-of-the-art methods.
\end{itemize}



==> method_bak.tex <==
\subsection{Overall Architecture}
\begin{figure}[tb]
\includegraphics[width=1\linewidth]{figs/overview_cropped.pdf}
\caption{An overview of the \ModelName. (1) The language model first extract textual feature sequence. (2) Our query-aware vision backbone extracts and fuse multiscale visual features with textual guidance. (3) The visual and textual feature sequences are fed into a transformer, and a [REG] token representation is used to regress the bounding box.}
\label{fig:model}
\end{figure}
% 介绍一下visual grounding的三个组件 提出vision backbone的两个问题semantic inconsistency and scale inconsistency
% 解决方法是使用linguistic feature guide visual feature extraction in vision backbone
% 讲一下介绍顺序 首先介绍我们引入的新颖的查询驱动的attention模块 再介绍如何基于此方法构建一个Modulated and Multiscale Swin-Transformer 以解决这两个问题
Before detailing the proposed mechanism and modules, we first present a typical visual grounding architecture used in this paper. We followed the recently proposed state-of-the-art architecture TransVG\cite{deng2021transvg}. Given an image and a query sentence, there is a linguistic backbone, typically a pre-trained BERT model, extracting a 1D feature sequence $t\in \mathbb{R}^{D_l\times N_l}$. There is also a vision backbone extracting a 2D feature map $v'\in \mathbb{R}^{D_v\times H\times W}$. Generally, the resolution of the feature map is $\frac{1}{2^s}$ of the origin image resolution, where $s$ is the number of downsample operators. The 2D feature map $v'$ is further flatten into a feature sequence $v \in \mathbb{R}^{D_v\times N_v}$, where $N_v=H\times W$. Two projection layers project the visual and linguistic features into the same feature space $\mathbb{R}^{D}$. The projected visual and linguistic features are denoted by $p_v\in \mathbb{R}^{D\times N_v}$ and $p_l\in \mathbb{R}^{D\times N_l}$. Then it concatenates $p_v$ and $p_l$ and inserts a learnable embedding (namely a [REG] token) at the begining of the concatenated sequence. The joint sequence is formulated as:
\begin{equation}
\begin{aligned}
\boldsymbol{x}_{0}=[p_{r}, \underbrace{p_{v}^{1}, p_{v}^{2}, \cdots, p_{v}^{N_{v}}}_{\text {visual tokens } \boldsymbol{p}_{v}}, \overbrace{p_{l}^{1}, p_{l}^{2}, \cdots, p_{l}^{N_{l}}}^{\text {linguistic tokens } p_{l}}]
\end{aligned}
\end{equation}
where $p^r$ is the learnable embedding of [REG] token.

A multi-layer visual-linguistic transformer with positional encoding is applied to perform inta- and inter- modal reasoning on the joint sequence. Finally, a prediction head takes the output representation of the [REG] token to predict the bounding box coordinates. Specifically, an MLP with ReLU activations transforms the $D$-dim [REG] embedding to 4-dim coordinates $b$. The smooth L1 loss and giou loss are using to train the framework. The training object can be formulated as:
\begin{equation}
\begin{aligned}
\mathcal{L}=\mathcal{L}_{smooth-l1}{(b,\hat{b})}+\mathcal{L}_{giou}{(b,\hat{b})}
\end{aligned}
\end{equation}
where $\hat{b}$ is the ground-truth box.

The structure of TransVG is elegant and representative of most visual grounding frameworks. We notice a widespread problem that not all visual signals in images are helpful for the grounding task. However, the vision backbone pre-trained on detection tasks tends to extract all objects it has learned. Moreover, the backbone is trained to extract features for classification and is not enough for cross-modal alignment. There is also a problem that the cross-modal interaction module takes the feature map from the last layer or a query-agnostic multi-scale fusion whose scale may be inconsistent with the referent object or be noisy.

To deal with these problems, we propose infusing the linguistic embedding into the vision backbone to guide the feature extraction and multi-scale feature fusion. To utilize the multi-scale feature, we first discard the vision backbone of TransVG because it only produces single-scale features. Instead, we use Swin-Transformer to extract multi-scale features. Then we introduce a novel Query-Driven Attention Mechanism, which leverages the linguistic embedding to drive the visual feature refinement. We further integrated the mechanism within the Swin-Transformer to guide the hierarchical feature extraction and multi-scale fusion. The improved backbone is called Modulated and Multiscale Swin-Transformer. We will cover the details in the following sections.

\subsection{Query-Driven Attention Mechanism}
In this section, we describe how we produce textual guidance and computing the visual attention distribution. Given an contextual textual representation $p_l^c \in \mathbb{R}^{D_l}$ (\eg a [CLS] token embedding), we introduce a Query Guidance Generator to generate a guide function $v_{clue}=G(v,\Theta_l)$. Then for each intermediate visual feature  map $v$. We use a Multi-level Feature Refinement module to produce a refined feature map $v^*=R(v,p_l^c)$ with the help of the decoder.%这里感觉需要根据示意图把方法流程大概过一遍 但这又和Multi-level Feature Refinement的过程比较近似

\subsubsection{Query Guidance Function}
The existing visual feature extractor uses modules with static parameters to process the visual feature map. For different data points with the same image, the outputs are the same. However, in visual grounding, the text reveals the intention of the query. For different query text, the crucial visual clues are also different.

Thus we propose a dynamic linear layer as our guidance function which parameters are decoded from the contextual textual representation $p_l^c$. For the guidance function, we define its parameters by $\Theta_l=\{W_l,b_l\},\,W_l\in \mathbb{R}^{D^{in}\times D^{out}},\, b_l\in \mathbb{R}^{D^{out}}$, where $D^{in}$ and $D^{out}$ are the dimensions of input and output respectively. The guidance function can be formulized as follow:
\begin{equation}
\begin{aligned}
v_{clue}&=G(v,\Theta_l)=vW_l+b_l
\end{aligned}
\end{equation}

A intuitive way to decode these parameters is introduce another larger linear module, which is denoted by $\Theta^{'}_l=\mathrm{Decoder}(p_l^c)$, where $\Theta^{'}_l\in\mathbb{R}^{(D^{in}+1)\ast D^{out}}$. We can simply reshape and split $\Theta^{'}_l$ to obtain $\{W_l,b_l\}$. However, it's easy to find that the number of parameters in the decoder is $D_l\ast ((D^{in}+1)\ast D^{out})$. We found that such large-scale parameters will slow down the training speed of the network and make it easier to be overfitting. Inspired by the application of matrix factorization, we consider decomposing the $\Theta_l$ into two factor $U\in \mathbb{R}^{(D^{in}+1)\times K}$ and $V\in \mathbb{R}^{K\times D^{out}}$, where $U$ is a matrix decoded from $p_l^c$, $V$ is a static learnable matrix, $K$ is a hyper-parameter denote the dimension of factor matrixes. The decompose-based decode $\{W_l,b_l\}=\mathrm{Decoder}^*(p_l^c)$ can be formulated as follow:
\begin{equation}
\begin{aligned}
U^{'} &= p_l^c W^{dec}+b^{dec}\\
U&=\mathrm{Reshape}(U^{'})
\end{aligned}
\end{equation}
where $W^{dec}\in \mathbb{R}^{D_l\times (D^{in}+1)\ast K}$ and $ b^{dec}\in \mathbb{R}^{(D^{in}+1)\ast K}$ are the paramemters of the factor decoder. We first use the factor decoder to calculate the vector $U^{'}\in \mathbb{R}^{(D^{in}+1)\ast K}$, We further reshape it into a matrix $U\in \mathbb{R}^{(D^{in}+1)\times K}$.
\begin{equation}
\begin{aligned}
\Theta_l&=UV\\
\{W_l,b_l\} &= \mathrm{Split}(\Theta_l)\\
\end{aligned}
\end{equation}
Then the parameter matrix of guidance function $\Theta_l$ can be reconstruct by multiply $U$ and $V$. The $W_l$ and $b_l$ can be split from the matrix $U$ along the first dimension. Finally, we reformulized the guidance function as follow:
\begin{equation}
\begin{aligned}
v_{clue}&=G^*(v,p_l^c)=G(v,\mathrm{Decoder}^*(p_l^c))
\end{aligned}
\end{equation}
%$p_l^c \in \mathbb{R}^{D_l},\, V\in \mathbb{R}^{K\times D^{out}},\, W^{dec}\in  \mathbb{R}^{D_l\times (D^{in}+1)\ast K},\, b^{dec}\in  \mathbb{R}^{(D^{in}+1)\ast K}$ backup the variable shape
\subsubsection{Multi-level Feature Refinement}
\begin{figure}[tb]
\centering
\includegraphics[width=1\linewidth]{figs/sc-attention_1_cropped.pdf}
\caption{Diagram of the Query-Driven Attention Mechanism}
\label{fig:query_attention}
\end{figure}

After obtaining the textual guidance, we consider refining the visual feature map. As explained earlier, the pre-trained vision backbone is sensitive to all salient objects. Most of them are irrelevant to the query text. Therefore, The backbone only needs to attend to a few areas. Besides, the extracted feature is suitable for the pretraining classification task instead of visual grounding. In other words, the importance of channels is different. Inspired by the Convolutional Block Attention Module\cite{woo2018cbam}, we consider infer a channel attention map $A_c$ to calibrate the semantic of feature for a better cross-modal alignment. And we further infer a spatial attention map $A_s$ from calibrated feature to reveal where the referent located.

Specifically, for a given visual feature $v\in \mathbb{R}^{H\times W\times D_v}$, we first aggregate its spatial information by average pooling and maximum pooling and produce $v^c_{max}\in \mathbb{R}^{1\times 1\times D_v}$ and $v^c_{mean}\in \mathbb{R}^{1\times 1\times D_v}$. We further build a query-driven multilayer perception (QMLP) consists of two guide functions. We use a ReLU activation after the first guide function. The output dimension is the same as the input dimension. To reduce the number of parameter, we set the dimension of hidden states as $D_v/r$, where $r$ is the reduction ratio. By feeding the $v^c_{max}$ and $v^c_{mean}$ to the QMLP, we merge the two output features using summation. The channel attention map $A_c$ can be captured as follow:
\begin{equation}
\begin{aligned}
v^{cl}_{mean}&=G^*_1(\mathrm{ReLU}(G^*_0(v^c_{mean},p_l^c)),p_l^c)\\
v^{cl}_{max}&=G^*_1(\mathrm{ReLU}(G^*_0(v^c_{max},p_l^c)),p_l^c)\\
A_c&=\mathrm{sigmoid}(v^{cl}_{mean}+v^{cl}_{max})
\end{aligned}
\end{equation}

We perform element-wise multiplication between $v$ and $A_c$ to form the representation of the channel refined visual feature:
\begin{equation}
\begin{aligned}
\dot{v}&=A_c\otimes v
\end{aligned}
\end{equation}

The $A_c$ are broadcast along the spatial dimension.

To generate a spatial attention map, instead pooling the channel dimension, we leverage a guidance function to reduce the channel dimension to learn areas interest to the query and apply a sigmoid function to generate the attention map. In short, The computing process is formulated as follow:
\begin{equation}
\begin{aligned}
A_s&=\mathrm{sigmoid}(G(\dot{v},p_l^c))\\
\ddot{v}&=A_c\otimes \dot{v}
\end{aligned}
\end{equation}
where $A_s\in \mathbb{R}^{H\times W\times 1}$ is the spatial attention map and $\ddot{v}$ is the spatial refined visual feature and also the output of our multi-level feature refinement.
\subsection{Modulated and Multiscale Swin-Transformer}
In this section, we discuss how to use query-driven attention to extend Swin-Transformer to a modulated vision backbone. We propose a Modulated Swin-Transformer Block to plug into each stage of Swin-Transformer architecture to help extract query-aware visual features. Thanks to the hierarchical structure, we can obtain features at different scales from each stage. We introduce a Query-guided Multiscale Feature Fusion to compute a scale-consist visual feature map. We present the proposed modules below.

\subsubsection{Modulated Swin-Transformer Block}
 For a given image $I \in \mathbb{R}^{H\times W\times 3}$, a plain Swin-Transformer first embed $I$ to a $v_0 \in \mathbb{R}^{\frac{H}{4}\times \frac{W}{4}\times 48}$. Then $v_0$ is feeded into four cascaded stages. Each stage $k$ receives the visual feature map $v_{k-1}$ and generates a transformed feature map $v_{k}$. As shown in \Cref{fig:stage}, we take the [CLS] representation of the input query sentence from BERT as the contextual query representation $p_l^c$. We append a Query-Driven Attention module after each Swin Transformer Block. It recieves the transformed feature $v_{k}$ and produces a query-aware feature $v_k^{*}$ to the next stage.
 \begin{figure}[tb]
\centering
\includegraphics[width=1\linewidth]{figs/block_cropped.pdf}
\caption{Modulated Swin-Transformer Block}
\label{fig:stage}
\end{figure}

\subsubsection{Query-guided Multiscale Feature Fusion}
\label{sec:multiscale}
Except the first stage, each stage reduce the resolution of feature map by a patch merging operator. In other words, the resolutions of the output of each stage are $\frac{H}{4}\times\frac{H}{4},\,\frac{H}{8}\times\frac{H}{8},\,\frac{H}{16}\times\frac{H}{16}$ and $\frac{H}{32}\times\frac{H}{32}$, respectively. Beside, the patch merging operator fuse the patch feature into channel which double the channel dimension. Thus the channel dimensions of the output of each stage are $C,\,2C,\,4C$ and $8C$.

Note that because visual grounding require fine-grained interaction (\eg Cross Attention), high-resolution features will dramatically increase the computation. Besides they will bring in noise and hurt the accuracy. Previous works using the last feature will obviously lose scale information. We propose to fuse the features with query guidance follow a bottom-up pathway. Specifically, we first use four $1\times 1$ convolutional layers to unify the channel dimensions to $D$. To filter out noisy signals in the feature maps, we build query-driven attention modules for the first three feature maps $\{v^{*}_k |\,k=1,2,3 \}$. Each module produce a weighted feature map with the same shape as before. Instead of interpolating the visual feature map to low-resolution, we consider apply a $2\times 2$ mean pooling with stride=2 to reduce the resolution to be the same as next feature map and add it to the next feature map $v^{*}_{k+1}$. Finally, the last feature map $v^{*}_{4}$ contains features interest to the query from all scales. We also apply a max pooling to obtain a smaller faeture map $v^{*}_{5} \in\frac{H}{64}\times\frac{H}{64}$. We flatten and concatenate the $v^{*}_{4}$ and $v^{*}_{5}$ as the output token sequence of our Modulated and Multiscale Swin-Transformer.
%可以说相对于stage内部的，这里的Query-Driven Attention挖掘的是适合grounding的尺度的特征 同时去除不适合的尺度信息。(不过没有实验支撑 看着说吧)
% 这里一定要强调 这里的query attention...可以达到选择尺度的作用，因为如果某个尺度的信息不重要，模型可以将其尺度的attention map设为0以避免其信息向下传。而Swin Transforme中的模块需要为预训练权重服务，如果靠前的特征的权重很低，则只有few feature被传递到之后的模块，因此只有少量预训练权重发挥了作用，模型性能会急剧降低，因此我们需要引入额外的多尺度聚合模块。




==> result.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}





% \multicolumn{11}{l}{Pre-training}  \\ 看要不要加在上面
% \begin{table*}[]
% \begin{tabular}{lcc}
% \hline
% \multicolumn{1}{c}{\multirow{2}{*}{Module}} & Flickr30K & \multicolumn{1}{l}{ReferItGame} \\
% \multicolumn{1}{c}{}                        & test      & test                            \\ \hline
% TransVG(SoTA)                               & 0.7910    & 0.7073                          \\
% Swin-Transformer(Baseline)                  & 0.7855    &                                 \\ \hline
% + Modulated Swin-Transformer Block          & 0.8116    & 0.7208                          \\ \hline
% \multicolumn{3}{l}{+ Query-guided Multiscale Feature Fusion}                              \\ \hline
% Attention-based Merge                       & 0.8143    & 0.7445                          \\
% Linear-based Merge                          & -         & \multicolumn{1}{l}{}            \\
% Gumbel Top-k Sample                         & 0.8109    & \multicolumn{1}{l}{}           
% \end{tabular}
% \end{table*}

==> revisit.tex <==
% 回顾一下End-to-end visual grounding的架构 引入需要将文本branch的信息注入到vision backbone中以获取文本感知的特征 以及需要基于文本从多尺度特征中进行选择。
